Adapting Multi-objectivized Software Configuration Tuning

When tuning software configuration for better performance (e.g., latency or throughput), an important issue that many optimizers face is the presence of local optimum traps, compounded by a highly rugged configuration landscape and expensive measurements. To mitigate these issues, a recent effort has shifted to focus on the level of optimization model (called meta multi-objectivization or MMO) instead of designing better optimizers as in traditional methods. This is done by using an auxiliary performance objective, together with the target performance objective, to help the search jump out of local optima. While effective, MMO needs a fixed weight to balance the two objectives-a parameter that has been found to be crucial as there is a large deviation of the performance between the best and the other settings. However, given the variety of configurable software systems, the "sweet spot" of the weight can vary dramatically in different cases and it is not possible to find the right setting without time-consuming trial and error. In this paper, we seek to overcome this significant shortcoming of MMO by proposing a weight adaptation method, dubbed AdMMO. Our key idea is to adaptively adjust the weight at the right time during tuning, such that a good proportion of the nondominated configurations can be maintained. Moreover, we design a partial duplicate retention mechanism to handle the issue of too many duplicate configurations without losing the rich information provided by the "good" duplicates. Experiments on several real-world systems, objectives, and budgets show that, for 71% of the cases, AdMMO is considerably superior to MMO and a wide range of state-of-the-art optimizers while achieving generally better efficiency with the best speedup between 2.2x and 20x.

==> figures/test/main-test.tex <==
\begin{figure*}[t!]
\centering

\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys1-avg}
\subcaption{vs. \textsc{IRACE}}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys2-avg}
\subcaption{vs. \textsc{GA}}
\end{subfigure}
\hspace{-0.4cm} 
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys3-avg}
\subcaption{vs. \textsc{RS}}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys4-avg}
\subcaption{vs. \textsc{ParamILS}}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys5-avg}
\subcaption{vs. \textsc{MMO}}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys6-avg}
\subcaption{vs. \textsc{PMO}}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys7-avg}
\subcaption{vs. \textsc{Flash}}
\end{subfigure}


\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys8-avg}
\subcaption{vs. \textsc{BOCA}}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys9-avg}
\subcaption{vs. \textsc{SMAC}}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys10-avg}
\subcaption{Maria-O1}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys11-avg}
\subcaption{Maria-O1}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys12-avg}
\subcaption{Maria-O1}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys13-avg}
\subcaption{Maria-O1}
\end{subfigure}
\hspace{-0.4cm}
\begin{subfigure}{.15\textwidth}
\includestandalone[width=\columnwidth]{figures/test/sys14-avg}
\subcaption{Maria-O1}
\end{subfigure}


\caption{The role of the maintained proportion of nondominated configurations ($p$) in AdMMO over 50 runs. (a) plots the best $p$ on each case; (b) shows the sensitivity during the tuning. The average and standard error of the normalized target performance objectives across all cases are reported. }
\label{fig:sen}
\end{figure*}

==> related.tex <==

% single objective (talk about jump out from local optima)
% mutiple objective
% PMO in other SBSE problem
% mreasurement  
% model based (including learning)
% 

\section{Related Work}
\label{sec:related}

We discuss the related work in light of AdMMO.

\textbf{\textit{Optimizers for Software Configuration Tuning}}:

Existing work 

\textbf{\textit{Optimizers for General Parameter Tuning}}:

\textbf{\textit{Multi-objectivization in SBSE}}:


\textbf{\textit{Measurement-based Optimizers:}} In measurement-based methods, the optimizer is directly used to measure the configuration on the software systems. Despite the expensiveness, the measurements can accurately reflect the good or bad of a configuration. The optimizer can be based on random search~\cite{DBLP:journals/jmlr/BergstraB12,DBLP:conf/sigmetrics/YeK03,DBLP:conf/sigsoft/OhBMS17}, hill climbing~\cite{DBLP:conf/www/XiLRXZ04,DBLP:conf/hpdc/LiZMTZBF14}, single-objective genetic algorithm~\cite{DBLP:conf/sc/BehzadLHBPAKS13,DBLP:conf/sigsoft/ShahbazianKBM20} and simulated annealing~\cite{DBLP:conf/icpads/DingLQ15,guo2010evaluating}, to name a few. Under such a single-objective model, various tricks have been applied. For example, some extend random search to consider a wider neighboring radius of the configuration structure, hence it is more likely to jump out from the local optima~\cite{DBLP:conf/sigsoft/OhBMS17}. Others rely on restarting from a different point, such as in restarted hill climbing, hence increasing the chance to find the ``right'' path from local optima to the global optimum~\cite{DBLP:conf/cloud/ZhuLGBMLSY17,DBLP:conf/www/XiLRXZ04}.

Our MMO model differs from all the above as it lies in a higher level of abstraction --- the optimization model --- as opposed to the level of optimization method. 
%The experiments have also shown that the purposely-crafted Pareto relation in MMO can overcome the local optima better for software configuration tuning. 
%\textcolor{red}{It may not be accurate to mention Pareto relation since we rely on the model, I have already commented the sentence out.}

%\subsection{Model-based Optimizers}

\textbf{\textit{Model-based Optimizers:}} Instead of solely using the measurements of software systems, the model-based methods apply a surrogate model (analytical~\cite{DBLP:conf/icse/Kumar0BB20,DBLP:conf/gecco/0001LY18,DBLP:journals/infsof/ChenLY19} or machine learning based~\cite{nair2018finding,DBLP:conf/mascots/JamshidiC16}) to evaluate configurations, which guides the search in an optimizer. The intention is to speed up the exploration of configurations as the model evaluation is rather cheap. Yet, it has been shown that the model accuracy and the availability of initial data can become an issue~\cite{DBLP:conf/cloud/ZhuLGBMLSY17}. Among others, Jamshidi and Casale~\cite{DBLP:conf/mascots/JamshidiC16} use Bayesian optimization to tune software configuration, wherein the search is guided by the Gaussian process regression trained from the data collected. Nair et al.~\cite{nair2018finding} follow a similar idea but a regression tree model is used instead.

Since MMO lies in the level of optimization model, it is complementary to the model-based methods in which the MMO would take the surrogate values as inputs instead of the real measurements.

%If the MMO model works with real measurements, which is the most accurate setting, then presumably the same applies to the model-based context where the search is guided by a surrogate value. \textcolor{red}{Working with accurate setting may not work with inaccurate setting?}


%\subsection{General Parameter Tuning}

\textbf{\textit{General Parameter Tuning:}} Optimizers proposed for the parameter tuning of general algorithms can also be relevant~\cite{DBLP:journals/ec/BlotMJH19,DBLP:journals/tec/HuangLY20,DBLP:series/sci/Bezerra0S20,DBLP:conf/ppsn/PushakH18}, including IRace~\cite{lopez2016irace}, ParamILS~\cite{DBLP:journals/jair/HutterHLS09}, SMAC~\cite{DBLP:conf/lion/HutterHL11}, GGA$++$~\cite{DBLP:conf/ijcai/AnsoteguiMSST15}, as well as their multi-objective variants, such as MO-ParamILS~\cite{DBLP:conf/lion/BlotHJKT16} and SPRINT-Race~\cite{DBLP:conf/gecco/ZhangGA15}. To examine a few examples, ParamILS~\cite{DBLP:journals/jair/HutterHLS09} relies on iterative local search --- a search procedure that may jump out of local optima using strategies similar to that of SA and SHC-r. Further, a key contribution is the capping strategy, which helps to reduce the need to measure an algorithm under some problem instances, hence saving computational resources. This is one of the goals that we seek to achieve too. Similar to Nair et al.~\cite{nair2018finding}, SMAC~\cite{DBLP:conf/lion/HutterHL11} uses Bayesian optimization but relying on a Random Forest model, which additionally considers the performance of an algorithms over a set of instances.

However, their work differs from ours in two aspects. 
	Firstly, general algorithm configuration requires to work on a set of problem instances, 
	each coming with different features. 
	The software configuration tuning, in contrast, is often concerned with tuning software system under a given benchmark (i.e., one instance)~\cite{nair2018finding,DBLP:conf/mascots/JamshidiC16,DBLP:conf/cloud/ZhuLGBMLSY17,Chen2018FEMOSAA}. Therefore, most of their designs for saving resources (such as the capping in ParamILS) were proposed to reduce the number of instances measured. Of course, it is possible to generalize the problem to consider multiple benchmarks as the same time, yet this is outside the scope of this paper. 
	Secondly, none of them works on the level of optimization model, and therefore our MMO is still complementary to their optimizers.




%\subsection{Multi-Objectivization in SBSE}

\textbf{\textit{Multi-Objectivization in SBSE:}} Multi-objectivization, which is the notion behind our MMO model, has been applied in other SBSE problems~\cite{DBLP:journals/tse/YuanB20,derakhshanfar2020good,DBLP:conf/ssbse/MkaouerKBC14,DBLP:conf/ssbse/SoltaniDPDZD18}. For example, to reproduce a crash based on the crash report, one can purposely design a new auxiliary objective, which measures how widely a test case covers the code, to be optimized alongside with the target crash distance~\cite{derakhshanfar2020good}. A multi-objective optimizer, e.g., NSGA-II, is directly used thereafter. A similar case can be found also for the code refactoring problem~\cite{DBLP:conf/ssbse/MkaouerKBC14}. However, during the tuning process, such a model, i.e., PMO in this paper, could waste a significant amount of the resources in optimizing the auxiliary objective, 
which is of no interest. 
This is a particularly unwelcome issue for software configuration tuning where the measurement is expensive. As we have shown in Section~\ref{sec:result}, PMO performs even worse than the classic single-objective model in most of the cases.


%Conceptually, this is resemble to existing multi-objective optimizers~\cite{Chen2018FEMOSAA,nair2018finding} for software configuration tuning, but without the assumption that all of the performance objectives are important.

%In summary, this work is, to the best of our knowledge, the first empirical study to understand whether, when, and why aspirations matter for guiding multi-objective software configuration tuning.


% single objective software configuration tuning

% multi objective software configuration tuning

% multi-objectivation in SBSE

% search based without aspiration, starting with single objective 
% search based with aspiration, starting with single objective
%(say with model and without)
% comparing weight vs Pareto, comparing reference point search, from SBSE or EC field

==> tables/all-bk.tex <==


% CS Table for RQ2
\begin{table*}[t!]
\caption{Comparing the optimizers on the average of normalized target performance over 50 runs (smaller value is preferred). The bottom-right shows the \% of statistically significant comparisons (and $\hat{A}_{12}$) against \textsc{AdMMO} over 56 cases. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} highlight the best in a case. The summarized raw results of all cases can be found at our anonymous repository: \url{https://github.com/3c23/admmo/blob/main/supp.pdf}.}
    \label{tb:rq1}
   % \footnotesize
    \setlength{\tabcolsep}{1mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     
   \begin{tabular}{l||l|llll||l|llll||l|llll||l|llll}
            \cellcolor[gray]{1}\textbf{Optimizer}  & \textbf{ID}& \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$} &\textbf{ID}& \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$} &\textbf{ID}& \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$} &\textbf{ID}& \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$}  \\
            \hline
            %&
            %\multicolumn{4}{c|}{\textsc{MariaDB-O1}}&
            %\multicolumn{4}{c|}{\textsc{MariaDB-O2}}&
            %\multicolumn{4}{c|}{\textsc{Storm-O1}}&
            %\multicolumn{4}{c}{\textsc{Storm-O2}}\\
            %\hline

\textsc{IRACE}&\multirow{10}{*}{$I_1$}&0.4774&0.3543&0.2813&0.2670&\multirow{10}{*}{$I_2$}&0.4933&0.3122&0.1673&0.1085&\multirow{10}{*}{$I_3$}&1.0000&0.6713&0.4944&0.3125&\multirow{10}{*}{$I_4$}&0.2317&0.1384&0.0932&0.0644\\
\textsc{GA}&&0.5061&0.1138&0.0867&0.0702&&0.2857&0.0715&0.0352&0.0091&&0.1671&0.0741&0.0571&0.0429&&\cellcolor{steel!30}0.0124&\cellcolor{steel!30}0.0024&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000\\
\textsc{RS}&&0.5172&0.3473&0.2468&0.1849&&0.4280&0.2812&0.2207&0.1343&&0.7768&0.4745&0.3254&0.2803&&0.1792&0.1169&0.0922&0.0692\\
\textsc{ParamILS}&&1.0000&0.5762&0.3904&0.1650&&1.0000&0.7029&0.5779&0.5326&&0.7240&0.4206&0.1829&0.0665&&1.0000&0.7186&0.3986&0.2560\\

\textsc{MMO}&&0.2166&0.1045&0.0712&0.0477&&\cellcolor{steel!30}0.2761&\cellcolor{steel!30}0.0589&0.0268&0.0052&&\cellcolor{steel!30}0.1173&0.0584&0.0435&0.0329&&0.0427&0.0016&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000\\

\textsc{PMO}&&0.5124&0.1573&0.0834&0.0515&&0.4505&0.3112&0.2365&0.1544&&0.6520&0.1887&0.0914&0.0480&&0.2813&0.0740&0.0216&0.0108\\

\textsc{Flash}&&0.4543&0.2270&0.1815&0.1657&&0.4979&0.0941&\cellcolor{steel!30}0.0033&\cellcolor{steel!30}0.0000&&0.8734&0.0481&0.0213&0.0058&&0.4423&0.0913&0.0913&0.0913\\

\textsc{BOCA}&&0.5545&0.3208&0.2437&0.1924&&0.4230&0.2808&0.2018&0.1897&&0.3323&0.1725&0.0928&0.0485&&0.2510&0.1325&0.0982&0.0814\\

\textsc{SMAC}&&0.5573&0.3956&0.3155&0.2699&&0.5258&0.3187&0.2214&0.1871&&0.9983&0.6810&0.4461&0.2944&&0.2198&0.1040&0.0768&0.0659\\

\textsc{AdMMO}&&\cellcolor{steel!30}0.2122&\cellcolor{steel!30}0.0531&\cellcolor{steel!30}0.0093&\cellcolor{steel!30}0.0000&&0.2823&0.1193&0.0654&0.0268&&0.1237&\cellcolor{steel!30}0.0299&\cellcolor{steel!30}0.0173&\cellcolor{steel!30}0.0000&&0.0416&0.0048&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000\\


\hline
\textsc{IRACE}&\multirow{10}{*}{$I_5$}&0.1069&0.0665&0.0436&0.0296&\multirow{10}{*}{$I_6$}&0.0486&0.0216&0.0181&0.0162&\multirow{10}{*}{$I_7$}&0.7580&0.6093&0.4898&0.3819&\multirow{10}{*}{$I_8$}&0.0696&0.0424&0.0366&0.0309\\

\textsc{GA}&&0.1315&0.0565&0.0246&0.0060&&0.0537&0.0230&0.0120&0.0075&&0.7959&0.6997&0.6501&0.6239&&0.0082&0.0033&0.0022&0.0019\\

\textsc{RS}&&0.1625&0.0625&0.0281&0.0240&&0.0587&0.0310&0.0237&0.0188&&0.8017&0.6706&0.5685&0.4927&&0.0799&0.0387&0.0281&0.0242\\

\textsc{ParamILS}&&1.0000&0.9901&0.9711&0.8899&&1.0000&0.9833&0.9773&0.8772&&1.0000&0.9913&0.9913&0.9854&&1.0000&0.6231&0.4191&0.3367\\

\textsc{MMO}&&0.1925&0.0512&0.0251&0.0004&&0.0831&0.0531&0.0425&0.0351&&0.8455&0.7638&0.6880&0.6122&&0.0068&0.0030&0.0020&0.0013\\

\textsc{PMO}&&0.1791&0.1021&0.0722&0.0519&&0.0820&0.0585&0.0438&0.0371&&\cellcolor{steel!30}0.2711&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000&&0.0128&0.0023&0.0017&0.0013\\

\textsc{Flash}&&0.1504&0.0647&0.0399&0.0162&&0.0503&0.0290&0.0208&0.0164&&0.9708&0.9708&0.9708&0.9708&&0.0799&0.0202&0.0186&0.0186\\

\textsc{BOCA}&&0.1627&0.0600&0.0459&0.0237&&0.0748&0.0428&0.0264&0.0172&&0.7580&0.6006&0.5510&0.4898&&0.0479&0.0280&0.0232&0.0193\\

\textsc{SMAC}&&0.1746&0.1004&0.0489&0.0259&&0.0530&0.0285&0.0211&0.0190&&0.7522&0.5685&0.5219&0.4490&&0.0601&0.0391&0.0334&0.0293\\

\textsc{AdMMO}&&\cellcolor{steel!30}0.0860&\cellcolor{steel!30}0.0451&\cellcolor{steel!30}0.0059&\cellcolor{steel!30}0.0000&&\cellcolor{steel!30}0.0447&\cellcolor{steel!30}0.0193&\cellcolor{steel!30}0.0034&\cellcolor{steel!30}0.0000&&0.7085&0.5569&0.4402&0.4169&&\cellcolor{steel!30}0.0059&\cellcolor{steel!30}0.0012&\cellcolor{steel!30}0.0003&\cellcolor{steel!30}0.0000\\



\hline


\textsc{IRACE}&\multirow{10}{*}{$I_9$}&0.5129&0.2621&0.1853&0.1013&\multirow{10}{*}{$I_{10}$}&0.4202&0.1947&0.1079&0.0809&\multirow{10}{*}{$I_{11}$}&0.3351&0.3351&0.3351&0.3351&\multirow{10}{*}{$I_{12}$}&0.0077&0.0077&0.0077&0.0077\\

\textsc{GA}&&0.5056&0.2795&0.1965&0.1041&&0.4777&0.2792&0.1536&0.0519&&0.1559&\cellcolor{steel!30}0.0487&0.0325&0.0179&&\cellcolor{steel!30}0.0029&0.0018&0.0015&0.0015\\

\textsc{RS}&&0.4724&0.2829&0.1900&0.1354&&0.4741&0.2624&0.1837&0.0642&&1.0000&1.0000&1.0000&1.0000&&0.0961&0.0961&0.0961&0.0961\\

\textsc{ParamILS}&&1.0000&1.0000&1.0000&1.0000&&1.0000&0.9936&0.9936&0.9936&&1.0000&1.0000&1.0000&1.0000&&1.0000&1.0000&1.0000&1.0000\\

\textsc{MMO}&&0.5541&0.3459&0.1746&0.0685&&0.4844&0.2831&0.1862&0.1185&&0.1918&0.0708&0.0214&\cellcolor{steel!30}0.0000&&0.0044&0.0016&0.0014&0.0011\\

\textsc{PMO}&&0.5140&0.2656&0.1681&0.0804&&0.4675&0.2236&0.1475&0.0604&&0.2510&0.1096&0.0574&0.0043&&0.0051&0.0021&0.0011&0.0007\\

\textsc{Flash}&&0.5821&0.3013&0.2191&0.1442&&0.4782&0.2191&0.1154&0.0803&&0.3351&0.3351&0.3351&0.3351&&0.0077&0.0077&0.0077&0.0077\\

\textsc{BOCA}&&0.6089&0.4453&0.2763&0.1810&&0.4570&0.2776&0.1724&0.1157&&0.3351&0.3351&0.3351&0.3351&&0.0077&0.0077&0.0077&0.0077\\

\textsc{SMAC}&&0.5709&0.3439&0.2264&0.1195&&0.5364&0.2590&0.1605&0.0931&&0.3351&0.3351&0.3351&0.3351&&0.0077&0.0077&0.0077&0.0077\\

\textsc{AdMMO}&&\cellcolor{steel!30}0.4332&\cellcolor{steel!30}0.1317&\cellcolor{steel!30}0.0361&\cellcolor{steel!30}0.0000&&\cellcolor{steel!30}0.3829&\cellcolor{steel!30}0.1611&\cellcolor{steel!30}0.0269&\cellcolor{steel!30}0.0000&&\cellcolor{steel!30}0.1424&0.0781&\cellcolor{steel!30}0.0194&0.0042&&0.0032&\cellcolor{steel!30}0.0012&\cellcolor{steel!30}0.0001&\cellcolor{steel!30}0.0000\\



%\cline{0-10}
\hline



\textsc{IRACE}&\multirow{10}{*}{$I_{13}$}&0.5210&0.4124&0.3804&0.3511&\multirow{10}{*}{$I_{14}$}&0.6465&0.4050&0.2831&0.2099&\multicolumn{2}{l}{\textbf{vs. Ours}}&\multicolumn{2}{c}{\textbf{trivial}}&\multicolumn{2}{c}{\textbf{small}}&\multicolumn{2}{c}{\textbf{medium}}&\multicolumn{2}{c}{\textbf{large}} \\

\cline{12-21}

\textsc{GA}&&\cellcolor{steel!30}0.0774&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000&&0.4918&0.2615&0.1821&0.1608&\multicolumn{2}{l}{\textsc{IRACE}}&\multicolumn{2}{c}{7\%}&\multicolumn{2}{c}{2\%}&\multicolumn{2}{c}{2\%}&\multicolumn{2}{c}{89\%} \\

\textsc{RS}&&0.5998&0.4709&0.4278&0.3937&&0.8072&0.5448&0.3880&0.2557&\multicolumn{2}{l}{\textsc{GA}}&\multicolumn{2}{c}{17\%}&\multicolumn{2}{c}{9\%}&\multicolumn{2}{c}{14\%}&\multicolumn{2}{c}{60\%} \\

\textsc{ParamILS}&&1.0000&0.9729&0.9510&0.9307&&1.0000&0.9191&0.8688&0.8171&\multicolumn{2}{l}{\textsc{RS}}&\multicolumn{2}{c}{2\%}&\multicolumn{2}{c}{5\%}&\multicolumn{2}{c}{2\%}&\multicolumn{2}{c}{91\%} \\

\textsc{MMO}&&0.0915&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000&&0.4876&0.2396&0.1680&0.1164&\multicolumn{2}{l}{\textsc{ParamILS}}&\multicolumn{2}{c}{0\%}&\multicolumn{2}{c}{0\%}&\multicolumn{2}{c}{4\%}&\multicolumn{2}{c}{96\%} \\

\textsc{PMO}&&0.2613&0.0956&0.0276&0.0155&&0.5450&0.3317&0.2534&0.2112&\multicolumn{2}{l}{\textsc{MMO}}&\multicolumn{2}{c}{16\%}&\multicolumn{2}{c}{9\%}&\multicolumn{2}{c}{21\%}&\multicolumn{2}{c}{54\%} \\

\textsc{Flash}&&0.4282&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000&&\cellcolor{steel!30}0.4651&0.2760&0.1306&0.0277&\multicolumn{2}{l}{\textsc{PMO}}&\multicolumn{2}{c}{4\%}&\multicolumn{2}{c}{5\%}&\multicolumn{2}{c}{11\%}&\multicolumn{2}{c}{80\%} \\

\textsc{BOCA}&&0.3971&0.3287&0.2961&0.2720&&0.7422&0.4786&0.3340&0.2130&\multicolumn{2}{l}{\textsc{Flash}}&\multicolumn{2}{c}{14\%}&\multicolumn{2}{c}{2\%}&\multicolumn{2}{c}{4\%}&\multicolumn{2}{c}{80\%} \\

\textsc{SMAC}&&0.5058&0.3888&0.3204&0.2910&&0.7112&0.4817&0.3210&0.2156&\multicolumn{2}{l}{\textsc{BOCA}}&\multicolumn{2}{c}{5\%}&\multicolumn{2}{c}{2\%}&\multicolumn{2}{c}{0\%}&\multicolumn{2}{c}{93\%} \\

\textsc{AdMMO}&&0.1156&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000&\cellcolor{steel!30}0.0000&&0.5216&\cellcolor{steel!30}0.2378&\cellcolor{steel!30}0.0984&\cellcolor{steel!30}0.0000&\multicolumn{2}{l}{\textsc{SMAC}}&\multicolumn{2}{c}{5\%}&\multicolumn{2}{c}{2\%}&\multicolumn{2}{c}{2\%}&\multicolumn{2}{c}{91\%} \\

\multicolumn{11}{c}{}&\multicolumn{10}{c}{\textbf{\% of significant cases vs. \textsc{AdMMO} over all 56 cases.}}\\

%\cline{0-10}

        \end{tabular}
        
  \end{adjustbox}
   \end{center}
   \vspace{-0.5cm}
\end{table*}




==> tables/all-old.tex <==


% CS Table for RQ2
\begin{table*}[t!]
\caption{Comparing MOO$+$ with the other state-of-the-arts over 50 runs. SO$_{best}$ and MMO$_{best}$ denote the best single-objective optimizer and the MMO model with the best weight, respectively. \quartexp{0}{20}{10}{20} shows the average and standard error on the target performance objective achieved (all objective values are normalized within $[0,1]$ and the closer to the left, the better). \bquartexp{0}{20}{10}{20} denote the best average among others. Column ``$\hat{A}_{12}$ ($p$ value)'' shows the $\hat{A}_{12}$ and $p$ value when comparing the corresponding counterpart with MOO$+$. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} denote MMO$+$ wins while \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red cells} mean it loses; otherwise it is a tie. The statistically significant comparisons, i.e., $\hat{A}_{12} \geq 0.56$ (or $\hat{A}_{12} \leq 0.44$) and $p<0.05$ are highlighted in bold.}
    \label{tb:rq1}
    \footnotesize
    %\setlength{\tabcolsep}{0.85mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     
   \begin{tabular}{l||l|llll||l|llll||l|llll||l|llll}
            \cellcolor[gray]{1}\textbf{Optimizer}  & \textbf{ID}& \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$} &\textbf{ID}& \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$} &\textbf{ID}& \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$} &\textbf{ID}& \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$}  \\
            \hline
            %&
            %\multicolumn{4}{c|}{\textsc{MariaDB-O1}}&
            %\multicolumn{4}{c|}{\textsc{MariaDB-O2}}&
            %\multicolumn{4}{c|}{\textsc{Storm-O1}}&
            %\multicolumn{4}{c}{\textsc{Storm-O2}}\\
            %\hline
\textsc{IRACE}&\multirow{10}{*}{O1}&0.3564&0.1771&0.1381&0.1219&\multirow{10}{*}{O2}& 0.617&0.3655&0.2363&0.1311&\multirow{10}{*}{O3}&0.7264&0.4757&0.3367&0.2346&\multirow{10}{*}{O4}&0.2451&0.1456&0.0941&0.0587  \\  
\textsc{GA}&&\cellcolor{steel!30}0.2523&0.1172&0.0514&0.0358&&\cellcolor{steel!30}0.4027&0.1403&0.0454&0.0321&&\cellcolor{steel!30}0.2628&0.0463&0.0372&0.0338&&\cellcolor{steel!30}0.0619&\cellcolor{steel!30}0.0024&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0\\  
\textsc{RS}&&0.7953&0.1857&0.1301&0.0933&&0.6751&0.3196&0.2424&0.1722&&1.0&0.3720&0.2286&0.1778&&0.9369&0.1234&0.0836&0.0621 \\ 
\textsc{ParamILS}&&1.0&0.2908&0.182&0.1217&&1.0&0.7255&0.6011&0.5283&&0.5405&0.3102&0.1593&0.0629&&1.0&0.7434&0.4091&0.2502 \\ 
\textsc{MMO}&&0.2812&0.0715&0.0417&0.0255&& 0.4417&\cellcolor{steel!30}0.1205&0.0308&0.0058&&0.3235&0.0360&0.0268&0.0228&&0.2619&0.0059&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0  \\ 
\textsc{PMO}&&0.4601&0.1490&0.0513&0.0329&&0.5767&0.3612&0.2908&0.2159&&0.7822&0.2014&0.0793&0.0377&&0.4435&0.1144&0.0335&0.0097 \\ 
\textsc{Flash}&&0.5648&0.1323&0.0916&0.0782&&0.6646&0.3281&\cellcolor{steel!30}0.0292&\cellcolor{steel!30}0.0&&0.9229&0.1829&0.0138&0.0072&&0.4625&0.2068&0.0759&0.0759 \\ 
\textsc{BOCA}&&0.6494&0.1840&0.1228&0.0993&& 0.6349&0.3238&0.2300&0.1894&&0.512&0.1414&0.0708&0.0415&& 0.6092&0.1503&0.097&0.0734  \\ 
\textsc{SMAC}&&0.6135&0.1901&0.1537&0.1255&&0.6349&0.3238&0.2300&0.1894&&0.8495&0.4751&0.3144&0.217&&0.3324&0.1240&0.0754&0.0599 \\ 
\textsc{AdMMO}&&0.3086&\cellcolor{steel!30}0.0428&\cellcolor{steel!30}0.0058&\cellcolor{steel!30}0.0&&0.4712&0.1757&0.0882&0.0432&&0.3675&\cellcolor{steel!30}0.0330&\cellcolor{steel!30}0.0131&\cellcolor{steel!30}0.0&&0.3029&0.0139&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0\\ 
\hline

\textsc{IRACE}&\multirow{10}{*}{O5}&0.3632&0.0796&0.0415&0.0316&\multirow{10}{*}{O6}& 0.2083&0.0326&0.0181&0.0157&\multirow{10}{*}{O7}&0.8196&0.6644&0.5521&0.4449&\multirow{10}{*}{O8}&0.1453&0.0370&0.0282&0.0236 \\  
\textsc{GA}&&0.2856&0.0714&0.0299&0.0032&&\cellcolor{steel!30}0.1517&0.0290&0.0155&0.0021&&0.8454&0.6376&0.5834&0.5671&&\cellcolor{steel!30}0.0452&0.0031&0.0018&0.0014 \\  
\textsc{RS}&&0.4512&0.105&0.0405&0.0222&&0.3220&0.0383&0.0247&0.0204&&1.0&0.9962&0.9912&0.9806&&0.8816&0.034&0.0234&0.0180 \\ 
\textsc{ParamILS}&&1.0&1.0&0.9882&0.8737&&1.0&1.0&0.9718&0.8974&&1.0&0.9962&0.9912&0.9806&&1.0&0.5335&0.3612&0.2849 \\ 
\textsc{MMO}&&0.4240&0.0788&0.0266&0.0038&& 0.1849&0.045&0.0228&0.0119&&0.8977&0.7602&0.6993&0.6598&&0.1591&0.0023&0.0018&0.0012 \\ 
\textsc{PMO}&&0.4022&0.1322&0.0928&0.0636&&0.2775&0.0706&0.0560&0.0468&&\cellcolor{steel!30}0.5438&\cellcolor{steel!30}0.0939&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0&&0.1638&0.0041&0.0015&0.0012 \\ 
\textsc{Flash}&&0.4431&0.1009&0.0438&0.0288&&0.2794&0.0360&0.0232&0.0174&&0.9638&0.9623&0.9623&0.9623&&0.1573&0.0370&0.0132&0.0132 \\ 
\textsc{BOCA}&&0.4102&0.1025&0.0421&0.0215&& 0.2713&0.0509&0.0296&0.0171&&0.8579&0.6488&0.5772&0.5143&&0.1457&0.0272&0.0178&0.0150 \\ 
\textsc{SMAC}&&0.4700&0.1332&0.0677&0.0228&&0.2910&0.0364&0.0219&0.0151&&0.8734&0.6375&0.5432&0.4757&&0.1771&0.0332&0.0254&0.0225 \\ 
\textsc{AdMMO}&&\cellcolor{steel!30}0.2811&\cellcolor{steel!30}0.0532&\cellcolor{steel!30}0.0262&\cellcolor{steel!30}0.0&&0.2324&\cellcolor{steel!30}0.0282&\cellcolor{steel!30}0.0122&\cellcolor{steel!30}0.0&&0.831&0.5658&0.4575&0.3811&&0.1949&\cellcolor{steel!30}0.0015&\cellcolor{steel!30}0.0003&\cellcolor{steel!30}0.0 \\

\hline


\textsc{IRACE}&\multirow{10}{*}{O9}&0.8662&0.728&0.2599&0.1398&\multirow{10}{*}{O10}&0.8973&0.69&0.2359&0.107&\multirow{10}{*}{O11}&0.3267&0.3267&0.3267&0.3267&\multirow{10}{*}{O12}&0.0077&0.0077&0.0077&0.0077 \\  
\textsc{GA}&&0.697&0.2697&0.1133&0.036&&0.7307&0.3592&0.2273&0.1368&&0.2448&0.0977&0.0399&0.0093&&0.0058&0.0022&0.0016&0.0014 \\  
\textsc{RS}&&0.7364&0.3557&0.2275&0.1747&&0.7307&0.3592&0.2273&0.1368&&1.0&1.0&1.0&1.0&&0.0961&0.0961&0.0961&0.0961 \\ 
\textsc{ParamILS}&&1.0&0.9934&0.9848&0.9848&&1.0&0.9808&0.9808&0.9808&&1.0&1.0&1.0&1.0&&1.0&1.0&1.0&1.0 \\ 
\textsc{MMO}&&0.7605&0.3117&0.1354&0.0508&& 0.6454&0.2438&0.1002&0.0354&&0.263&0.1168&0.0389&0.0004&&0.0061&0.0027&0.0014&0.0012 \\ 
\textsc{PMO}&&\cellcolor{steel!30}0.6363&0.2572&0.1233&0.0483&&0.6359&0.2362&0.1148&0.0468&&0.2882&0.1571&0.0675&0.0104&&0.0069&0.0034&0.0015&0.0008 \\ 
\textsc{Flash}&&0.7279&0.3023&0.1749&0.1211&&0.6483&0.2665&0.152&0.1152&&0.3267&0.3267&0.3267&0.3267&&0.0077&0.0077&0.0077&0.0077 \\ 
\textsc{BOCA}&&0.7567&0.3887&0.238&0.1698&&\cellcolor{steel!30}0.6082&0.2659&0.1802&0.1337&&0.3267&0.3267&0.3267&0.3267&&0.0077&0.0077&0.0077&0.0077 \\ 
\textsc{SMAC}&&0.7168&0.2972&0.2052&0.1354&&0.6946&0.2463&0.175&0.1107&&0.3267&0.3267&0.3267&0.3267&&0.0077&0.0077&0.0077&0.0077 \\ 
\textsc{AdMMO}&&0.6736&\cellcolor{steel!30}0.1834&\cellcolor{steel!30}0.0601&\cellcolor{steel!30}0.0&&0.6596&\cellcolor{steel!30}0.2237&\cellcolor{steel!30}0.0768&\cellcolor{steel!30}0.0&&\cellcolor{steel!30}0.2304&\cellcolor{steel!30}0.0963&\cellcolor{steel!30}0.0375&\cellcolor{steel!30}0.0&&\cellcolor{steel!30}0.0057&\cellcolor{steel!30}0.0021&\cellcolor{steel!30}0.0004&\cellcolor{steel!30}0.0 \\


%\cline{0-10}
\hline

\textsc{IRACE}&\multirow{10}{*}{O13}&0.6403&0.467&0.4063&0.3715&\multirow{10}{*}{O14}&0.6955&0.4309&0.2509&0.1679&\multicolumn{1}{c}{}&&&&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&&& \\
\textsc{GA}&&\cellcolor{steel!30}0.3027&\cellcolor{steel!30}0.0072&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0&&\cellcolor{steel!30}0.6033&0.2535&0.1433&0.1148&\multicolumn{1}{c}{}&&&&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&&& \\  
\textsc{RS}&&0.7889&0.522&0.451&0.411&&1.0&0.5444&0.35&0.2385&\multicolumn{1}{c}{}&&&&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&&& \\
\textsc{ParamILS}&&0.9901&0.9941&1.0&0.9289&&0.9641&0.7999&0.729&0.6901&\multicolumn{1}{c}{}&&&&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&&& \\ 
\textsc{MMO}&&0.4171&0.0113&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0&&0.7639&\cellcolor{steel!30}0.2434&0.1412&0.0727&\multicolumn{1}{c}{}&&&&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&&& \\
\textsc{PMO}&&0.5597&0.1333&0.0226&0.0080&&0.7664&0.3168&0.2413&0.2041&\multicolumn{1}{c}{}&&&&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&&& \\
\textsc{Flash}&&0.5916&0.1633&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0&&0.6259&0.2537&0.1399&0.017&\multicolumn{1}{c}{}&&&&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&&& \\
\textsc{BOCA}&&0.5238&0.3609&0.3099&0.2852&& 0.8137&0.4896&0.3131&0.2054&\multicolumn{1}{c}{}&&&&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&&& \\ 
\textsc{SMAC}&&0.6271&0.4314&0.3487&0.3148&&0.8003&0.4754&0.3087&0.2118&\multicolumn{1}{c}{}&&&&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&&& \\
\textsc{AdMMO}&&0.407&0.0248&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0&&0.7165&0.2962&\cellcolor{steel!30}0.0894&\cellcolor{steel!30}0.0&\multicolumn{1}{c}{}&&&&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&&& \\

\cline{0-10}

        \end{tabular}
        
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/bk.tex <==


% CS Table for RQ2
\begin{table*}[t!]
\caption{Comparing MOO$+$ with the other state-of-the-arts over 50 runs. SO$_{best}$ and MMO$_{best}$ denote the best single-objective optimizer and the MMO model with the best weight, respectively. \quartexp{0}{20}{10}{20} shows the average and standard error on the target performance objective achieved (all objective values are normalized within $[0,1]$ and the closer to the left, the better). \bquartexp{0}{20}{10}{20} denote the best average among others. Column ``$\hat{A}_{12}$ ($p$ value)'' shows the $\hat{A}_{12}$ and $p$ value when comparing the corresponding counterpart with MOO$+$. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} denote MMO$+$ wins while \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red cells} mean it loses; otherwise it is a tie. The statistically significant comparisons, i.e., $\hat{A}_{12} \geq 0.56$ (or $\hat{A}_{12} \leq 0.44$) and $p<0.05$ are highlighted in bold.}
    \label{tb:rq1}
    \footnotesize
    %\setlength{\tabcolsep}{0.85mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     
   \begin{tabular}{llllll|lllll|lllll|lllll}
            \cellcolor[gray]{1}\textbf{}  & & \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$} & \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$} & \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$} & \cellcolor[gray]{1}\textbf{$S_{100}$} & \cellcolor[gray]{1}\textbf{$S_{200}$} & \cellcolor[gray]{1}\textbf{$S_{300}$} & \cellcolor[gray]{1}\textbf{$S_{400}$}  \\
            \hline
            %&
            %\multicolumn{4}{c|}{\textsc{MariaDB-O1}}&
            %\multicolumn{4}{c|}{\textsc{MariaDB-O2}}&
            %\multicolumn{4}{c|}{\textsc{Storm-O1}}&
            %\multicolumn{4}{c}{\textsc{Storm-O2}}\\
            %\hline
\textsc{IRACE}&\multirow{10}{*}{O1}&0.3564&0.1771&0.1381&0.1219&\multirow{10}{*}{O2} 0.617&0.3655&0.2363&0.1311&\multirow{10}{*}{O3}0.7264&0.4757&0.3367&0.2346&\multirow{10}{*}{O4}0.2451&0.1456&0.0941&0.0587  \\  
\textsc{GA}&&\cellcolor{steel!30}0.2523&0.1172&0.0514&0.0358&&\cellcolor{steel!30}0.4027&0.1403&0.0454&0.0321&&\cellcolor{steel!30}0.2628&0.0463&0.0372&0.0338&&\cellcolor{steel!30}0.0619&\cellcolor{steel!30}0.0024&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0\\  
\textsc{RS}&&0.7953&0.1857&0.1301&0.0933&&0.6751&0.3196&0.2424&0.1722&&1.0&0.3720&0.2286&0.1778&0.9369&&0.1234&0.0836&0.0621 \\ 
\textsc{ParamILS}&&1.0&0.2908&0.182&0.1217&&1.0&0.7255&0.6011&0.5283&&0.5405&0.3102&0.1593&0.0629&&1.0&0.7434&0.4091&0.2502 \\ 
\textsc{MMO}&&0.2812&0.0715&0.0417&0.0255&& 0.4417&\cellcolor{steel!30}0.1205&0.0308&0.0058&&0.3235&0.0360&0.0268&0.0228&&0.2619&0.0059&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0  \\ 
\textsc{PMO}&&0.4601&0.1490&0.0513&0.0329&&0.5767&0.3612&0.2908&0.2159&&0.7822&0.2014&0.0793&0.0377&&0.4435&0.1144&0.0335&0.0097 \\ 
\textsc{Flash}&&0.5648&0.1323&0.0916&0.0782&&0.6646&0.3281&\cellcolor{steel!30}0.0292&\cellcolor{steel!30}0.0&&0.9229&0.1829&0.0138&0.0072&&0.4625&0.2068&0.0759&0.0759 \\ 
\textsc{BOCA}&&0.6494&0.1840&0.1228&0.0993&& 0.6349&0.3238&0.2300&0.1894&&0.512&0.1414&0.0708&0.0415&& 0.6092&0.1503&0.097&0.0734  \\ 
\textsc{SMAC}&&0.6135&0.1901&0.1537&0.1255&&0.6349&0.3238&0.2300&0.1894&&0.8495&0.4751&0.3144&0.217&&0.3324&0.1240&0.0754&0.0599 \\ 
\textsc{AdMMO}&&0.3086&\cellcolor{steel!30}0.0428&\cellcolor{steel!30}0.0058&\cellcolor{steel!30}0.0&&0.4712&0.1757&0.0882&0.0432&0.3675&&\cellcolor{steel!30}0.0330&\cellcolor{steel!30}0.0131&\cellcolor{steel!30}0.0&&0.3029&0.0139&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0\\ 
\hline

 &
            \multicolumn{4}{c|}{\textsc{VP9-O1}}&
            \multicolumn{4}{c|}{\textsc{VP9-O2}}&
            \multicolumn{4}{c|}{\textsc{Keras-O1}}&
            \multicolumn{4}{c}{\textsc{Keras-O2}}\\
            \hline
\textsc{IRACE}&0.3632&0.0796&0.0415&0.0316& 0.2083&0.0326&0.0181&0.0157&0.8196&0.6644&0.5521&0.4449& 0.1453&0.0370&0.0282&0.0236 \\  
\textsc{GA}&0.2856&0.0714&0.0299&0.0032&\cellcolor{steel!30}0.1517&0.0290&0.0155&0.0021&0.8454&0.6376&0.5834&0.5671&\cellcolor{steel!30}0.0452&0.0031&0.0018&0.0014 \\  
\textsc{RS}&0.4512&0.105&0.0405&0.0222&0.3220&0.0383&0.0247&0.0204&1.0&0.9962&0.9912&0.9806&0.8816&0.034&0.0234&0.0180 \\ 
\textsc{ParamILS}&1.0&1.0&0.9882&0.8737&1.0&1.0&0.9718&0.8974&1.0&0.9962&0.9912&0.9806&1.0&0.5335&0.3612&0.2849 \\ 
\textsc{MMO}&0.4240&0.0788&0.0266&0.0038& 0.1849&0.045&0.0228&0.0119&0.8977&0.7602&0.6993&0.6598&0.1591&0.0023&0.0018&0.0012 \\ 
\textsc{PMO}&0.4022&0.1322&0.0928&0.0636&0.2775&0.0706&0.0560&0.0468&\cellcolor{steel!30}0.5438&\cellcolor{steel!30}0.0939&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0&0.1638&0.0041&0.0015&0.0012 \\ 
\textsc{Flash}&0.4431&0.1009&0.0438&0.0288&0.2794&0.0360&0.0232&0.0174&0.9638&0.9623&0.9623&0.9623&0.1573&0.0370&0.0132&0.0132 \\ 
\textsc{BOCA}&0.4102&0.1025&0.0421&0.0215& 0.2713&0.0509&0.0296&0.0171&0.8579&0.6488&0.5772&0.5143&0.1457&0.0272&0.0178&0.0150 \\ 
\textsc{SMAC}&0.4700&0.1332&0.0677&0.0228&0.2910&0.0364&0.0219&0.0151&0.8734&0.6375&0.5432&0.4757&0.1771&0.0332&0.0254&0.0225 \\ 
\textsc{AdMMO}&\cellcolor{steel!30}0.2811&\cellcolor{steel!30}0.0532&\cellcolor{steel!30}0.0262&\cellcolor{steel!30}0.0&0.2324&\cellcolor{steel!30}0.0282&\cellcolor{steel!30}0.0122&\cellcolor{steel!30}0.0&0.831&0.5658&0.4575&0.3811&0.1949&\cellcolor{steel!30}0.0015&\cellcolor{steel!30}0.0003&\cellcolor{steel!30}0.0 \\

\hline

 &
            \multicolumn{4}{c|}{\textsc{MongoDB-O1}}&
            \multicolumn{4}{c|}{\textsc{MongoDB-O2}}&
            \multicolumn{4}{c|}{\textsc{x264-O1}}&
            \multicolumn{4}{c}{\textsc{x264-O2}}\\
            \hline
\textsc{IRACE}&0.8662&0.728&0.2599&0.1398&0.8973&0.69&0.2359&0.107&0.4693&0.4693&0.4693&0.4693&0.0077&0.0077&0.0077&0.0077 \\  
\textsc{GA}&0.697&0.2697&0.1133&0.036&0.7307&0.3592&0.2273&0.1368&0.4047&0.2827&0.2354&0.2191&0.0058&0.0022&0.0016&0.0014 \\  
\textsc{RS}&0.7364&0.3557&0.2275&0.1747&0.7307&0.3592&0.2273&0.1368&1.0&1.0&1.0&1.0&0.0961&0.0961&0.0961&0.0961 \\ 
\textsc{ParamILS}&1.0&0.9934&0.9848&0.9848&1.0&0.9808&0.9808&0.9808&1.0&1.0&1.0&1.0&1.0&1.0&1.0&1.0 \\ 
\textsc{MMO}&0.7605&0.3117&0.1354&0.0508& 0.6454&0.2438&0.1002&0.0354&0.4191&0.3039&0.2409&0.2118&0.0061&0.0027&0.0014&0.0012 \\ 
\textsc{PMO}&\cellcolor{steel!30}0.6363&0.2572&0.1233&0.0483&0.6359&0.2362&0.1148&0.0468&0.4389&0.3356&0.2649&0.22&0.0069&0.0034&0.0015&0.0008 \\ 
\textsc{Flash}&0.7279&0.3023&0.1749&0.1211&0.6483&0.2665&0.152&0.1152&0.3263&0.3258&0.3258&0.3258&0.0136&0.0135&0.0135&0.0135 \\ 
\textsc{BOCA}&0.7567&0.3887&0.238&0.1698&\cellcolor{steel!30}0.6082&0.2659&0.1802&0.1337&0.0024&0.0011&0.0090&0.0&0.0067&0.0066&0.0066&0.0066 \\ 
\textsc{SMAC}&0.7168&0.2972&0.2052&0.1354&0.6946&0.2463&0.175&0.1107&0.3383&0.336&0.336&0.336&0.0134&0.0132&0.0132&0.0132 \\ 
\textsc{AdMMO}&0.6736&\cellcolor{steel!30}0.1834&\cellcolor{steel!30}0.0601&\cellcolor{steel!30}0.0&0.6596&\cellcolor{steel!30}0.2237&\cellcolor{steel!30}0.0768&\cellcolor{steel!30}0.0&0.3934&0.2876&0.2413&0.2118&\cellcolor{steel!30}0.0057&\cellcolor{steel!30}0.0021&\cellcolor{steel!30}0.0004&\cellcolor{steel!30}0.0 \\

\cline{0-8}

 &
            \multicolumn{4}{c|}{\textsc{LLVM-O1}}&
            \multicolumn{4}{c|}{\textsc{LLVM-O2}}&
            \multicolumn{4}{c}{}&
            \multicolumn{4}{c}{}\\
            \cline{0-8}
\textsc{IRACE}&0.6403&0.467&0.4063&0.3715&0.6955&0.4309&0.2509&0.1679&&&&\multicolumn{1}{c}{}&&& \\
\textsc{GA}&\cellcolor{steel!30}0.3027&\cellcolor{steel!30}0.0072&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.6033&0.2535&0.1433&0.1148&&&&\multicolumn{1}{c}{}&&& \\  
\textsc{RS}&0.7889&0.522&0.451&0.411&1.0&0.5444&0.35&0.2385&&&&\multicolumn{1}{c}{}&&& \\
\textsc{ParamILS}&0.9901&0.9941&1.0&0.9289&0.9641&0.7999&0.729&0.6901&&&&\multicolumn{1}{c}{}&&& \\ 
\textsc{MMO}&0.4171&0.0113&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0&0.7639&\cellcolor{steel!30}0.2434&0.1412&0.0727&&&&\multicolumn{1}{c}{}&&& \\
\textsc{PMO}&0.5597&0.1333&0.0226&0.0080&0.7664&0.3168&0.2413&0.2041&&&&\multicolumn{1}{c}{}&&& \\
\textsc{Flash}&0.5916&0.1633&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0&0.6259&0.2537&0.1399&0.017&&&&\multicolumn{1}{c}{}&&& \\
\textsc{BOCA}&0.5238&0.3609&0.3099&0.2852& 0.8137&0.4896&0.3131&0.2054&&&&\multicolumn{1}{c}{}&&& \\ 
\textsc{SMAC}&0.6271&0.4314&0.3487&0.3148&0.8003&0.4754&0.3087&0.2118&&&&\multicolumn{1}{c}{}&&& \\
\textsc{AdMMO}&0.407&0.0248&\cellcolor{steel!30}0.0&\cellcolor{steel!30}0.0&0.7165&0.2962&\cellcolor{steel!30}0.0894&\cellcolor{steel!30}0.0&&&&\multicolumn{1}{c}{}&&& \\

        \end{tabular}
        
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/rq1-1.tex <==


% CS Table for RQ2
\begin{table*}[t!]
\caption{Comparing AdMOO with the state-of-the-art measurement-based optimizers over 50 runs. \quartexp{0}{20}{10}{20} denotes the average and standard error (SE) on the normalized target performance objective achieved (the closer to the left, the better). \bquartexp{0}{20}{10}{20} denotes the best average among others. Column ``$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})'' shows the $\mathbf{\hat{A}_{12}}$ and \textbf{p-value} when comparing the corresponding optimizer with AdMOO. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} and \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red cells} denote AdMMO wins ($\mathbf{\hat{A}_{12}}>0.5$) and loses ($\mathbf{\hat{A}_{12}}<0.5$), respectively; otherwise it is a tie ($\mathbf{\hat{A}_{12}}=0.5$). The statistically significant comparisons, i.e., $\mathbf{\hat{A}_{12}} \geq 0.56$ (or $\mathbf{\hat{A}_{12}} \leq 0.44$) and \textit{p-value} $<0.05$ are highlighted in bold. Tables of raw results throughout the tuning can be found at: \href{https://github.com/3c23/admmo/blob/main/supp-data.pdf}{\texttt{\textcolor{blue}{https://github.com/3c23/admmo/blob/main/supp-data.pdf}}}.}
    \label{tb:rq1-1}
    \footnotesize
    \setlength{\tabcolsep}{0.85mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc@{}cc}
   % \toprule
        \begin{tabular}{l|c|cc}
            \cellcolor[gray]{1}\textbf{} &\textbf{} & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


IRACE&\multirow{7}{*}{\rotatebox{90}{\textsc{MariaDB-O1}}}&\cellcolor{steel!30}\textbf{.88 ($<$.001)}& \quart{82.19}{17.81}{91.09}{100} \\ 
GA&&\cellcolor{steel!30}\textbf{.68 ($=$.002)}& \quart{21.97}{10.46}{27.20}{100} \\ 
RS&&\cellcolor{steel!30}\textbf{.86 ($<$.001)}& \quart{58.00}{12.89}{64.44}{100} \\ 
MMO&&\cellcolor{steel!30}\textbf{.62 ($=$.041)}& \quart{14.63}{10.49}{19.87}{100} \\ 
PMO&&\cellcolor{steel!30}\textbf{.64 ($=$.018)}& \quart{15.60}{11.06}{21.13}{100} \\ 
AdMMO&&-& \bquart{0.00}{8.79}{4.40}{100} \\ 
&&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
         \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


\multirow{7}{*}{\rotatebox{90}{\textsc{MariaDB-O2}}}&\cellcolor{steel!30}{.58 ($=$.194)}& \quart{48.00}{26.89}{61.44}{100} \\ 
&\cellcolor{red!10}{.42 ($=$.166)}& \quart{2.53}{13.24}{9.15}{100} \\ 
&\cellcolor{steel!30}\textbf{.68 ($=$.002)}& \quart{62.23}{25.60}{75.03}{100} \\ 
&\cellcolor{red!10}{.43 ($=$.210)}& \bquart{0.00}{14.26}{7.13}{100} \\ 
&\cellcolor{steel!30}\textbf{.67 ($=$.004)}& \quart{71.16}{28.84}{85.58}{100} \\ 
&-& \quart{12.76}{11.47}{18.49}{100} \\ 
&&\squart{1}{1}{1}{100}\\   

        \end{tabular} &
        &
       \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


\multirow{7}{*}{\rotatebox{90}{\textsc{Storm-O1}}}&\cellcolor{steel!30}\textbf{.83 ($<$.001)}& \quart{74.62}{25.38}{87.31}{100} \\ 
&\cellcolor{steel!30}\textbf{.75 ($<$.001)}& \quart{9.50}{3.27}{11.13}{100} \\ 
&\cellcolor{steel!30}\textbf{.86 ($<$.001)}& \quart{68.19}{20.09}{78.23}{100} \\ 
&\cellcolor{steel!30}\textbf{.69 ($=$.001)}& \quart{6.81}{3.15}{8.39}{100} \\ 
&\cellcolor{steel!30}\textbf{.86 ($<$.001)}& \quart{11.48}{2.34}{12.65}{100} \\ 
&-& \bquart{0.00}{1.47}{0.73}{100} \\ 

&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


\multirow{7}{*}{\rotatebox{90}{\textsc{Storm-O2}}}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}& \quart{78.23}{13.01}{84.73}{100} \\ 
&{.50 ($=$1.00)}& \bquart{0.00}{0.00}{0.00}{100} \\ 
&\cellcolor{steel!30}\textbf{.97 ($<$.001)}& \quart{82.03}{17.97}{91.02}{100} \\ 
&{.50 ($=$1.00)}& \bquart{0.00}{0.00}{0.00}{100} \\ 
&\cellcolor{steel!30}{.59 ($=$.121)}& \quart{8.21}{11.95}{14.18}{100} \\ 
&-& \bquart{0.00}{0.00}{0.00}{100} \\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
     \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline

%&\cellcolor{steel!30}\textbf{.98 ($<$.001)}& \quart{30.91}{26.09}{43.96}{100} \\ 
%&\cellcolor{steel!30}\textbf{.67 ($=$.003)}& \quart{0.54}{0.24}{0.66}{100} \\ 
%&\cellcolor{steel!30}\textbf{.98 ($<$.001)}& \quart{24.67}{21.86}{35.60}{100} \\ 
%&\cellcolor{steel!30}\textbf{.64 ($=$.018)}& \quart{0.46}{0.26}{0.59}{100} \\ 
%&\cellcolor{steel!30}\textbf{.87 ($<$.001)}& \quart{53.96}{46.04}{76.98}{100} \\ 
%&-& \bquart{0.00}{0.24}{0.12}{100} \\ 


\multirow{7}{*}{\rotatebox{90}{\textsc{VP-O1}}}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}& \quart{30.96}{26.08}{43.99}{100} \\ 
&\cellcolor{steel!30}\textbf{.73 ($<$.001)}& \quart{0.93}{16.15}{9.00}{100} \\ 
&\cellcolor{steel!30}\textbf{.99 ($<$.001)}& \quart{24.72}{21.84}{35.64}{100} \\ 
&\cellcolor{steel!30}\textbf{.65 ($=$.009)}& \quart{0.53}{0.26}{0.66}{100} \\ 
&\cellcolor{steel!30}\textbf{.88 ($<$.001)}& \quart{53.99}{46.01}{76.99}{100} \\ 
&-& \bquart{0.00}{0.23}{0.11}{100} \\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular}  


   \vspace{0.05cm}
        \\ \midrule

        
        
              \begin{tabular}{l|c|x{1.4cm}c}


IRACE&\multirow{7}{*}{\rotatebox{90}{\textsc{VP-O2}}}&\cellcolor{steel!30}\textbf{.78 ($<$.001)}& \quart{23.20}{4.93}{25.66}{100} \\ 
GA&&{.50 ($=$.945)}& \bquart{0.00}{1.77}{0.89}{100} \\ 
RS&&\cellcolor{steel!30}\textbf{.84 ($<$.001)}& \quart{27.93}{3.64}{29.75}{100} \\ 
MMO&&\cellcolor{steel!30}{.54 ($=$.493)}& \quart{9.35}{90.65}{54.68}{100} \\ 
PMO&&\cellcolor{steel!30}\textbf{.80 ($<$.001)}& \quart{49.83}{15.81}{57.74}{100} \\ 
AdMMO&&-& \quart{7.34}{10.08}{12.38}{100} \\ 
&&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
            \begin{tabular}{|c|x{1.4cm}c}

\multirow{7}{*}{\rotatebox{90}{\textsc{Keras-O1}}}&\cellcolor{red!10}{.47 ($=$.588)}& \quart{48.05}{16.95}{56.52}{100} \\ 
&\cellcolor{steel!30}\textbf{.62 ($=$.043)}& \quart{84.66}{15.34}{92.33}{100} \\ 
&\cellcolor{steel!30}{.55 ($=$.426)}& \quart{63.87}{18.10}{72.91}{100} \\ 
&\cellcolor{steel!30}{.61 ($=$.067)}& \quart{83.13}{14.95}{90.60}{100} \\ 
&\cellcolor{red!10}\textbf{.25 ($<$.001)}& \bquart{0.00}{0.00}{0.00}{100} \\ 
&-& \quart{52.79}{17.81}{61.70}{100} \\ 

&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
            \begin{tabular}{|c|x{1.4cm}c}
  


\multirow{7}{*}{\rotatebox{90}{\textsc{Keras-O2}}}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}& \quart{79.59}{20.41}{89.80}{100} \\ 
&\cellcolor{steel!30}\textbf{.76 ($<$.001)}& \quart{5.07}{1.48}{5.81}{100} \\ 
&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}& \quart{64.17}{12.50}{70.42}{100} \\ 
&\cellcolor{steel!30}\textbf{.67 ($=$.003)}& \quart{3.46}{1.58}{4.25}{100} \\ 
&\cellcolor{steel!30}\textbf{.70 ($<$.001)}& \quart{3.59}{1.28}{4.23}{100} \\ 
&-& \bquart{0.00}{0.91}{0.46}{100} \\ 

&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
              \begin{tabular}{|c|x{1.4cm}c}



%&\cellcolor{steel!30}\textbf{.73 ($<$.001)}& \quart{49.15}{30.46}{64.38}{100} \\ 
%&\cellcolor{steel!30}\textbf{.63 ($=$.023)}& \quart{25.92}{41.33}{46.58}{100} \\ 
%&\cellcolor{steel!30}\textbf{.78 ($<$.001)}& \quart{63.80}{36.20}{81.90}{100} \\ 
%&\cellcolor{steel!30}\textbf{.64 ($=$.018)}& \quart{27.91}{39.22}{47.52}{100} \\ 
%&\cellcolor{steel!30}\textbf{.64 ($=$.017)}& \quart{33.33}{40.55}{53.61}{100} \\ 
%&-& \bquart{0.00}{33.78}{16.89}{100} \\ 

\multirow{7}{*}{\rotatebox{90}{\textsc{MongoDB-O1}}}&\cellcolor{steel!30}\textbf{.75 ($<$.001)}& \quart{51.57}{29.01}{66.08}{100} \\ 
&\cellcolor{steel!30}\textbf{.69 ($=$.001)}& \quart{45.70}{43.49}{67.44}{100} \\ 
&\cellcolor{steel!30}\textbf{.81 ($<$.001)}& \quart{65.52}{34.48}{82.76}{100} \\ 
&\cellcolor{steel!30}\textbf{.68 ($=$.002)}& \quart{31.34}{37.35}{50.02}{100} \\ 
&\cellcolor{steel!30}\textbf{.67 ($=$.003)}& \quart{36.51}{38.62}{55.81}{100} \\ 
&-& \bquart{0.00}{32.97}{16.48}{100} \\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
            \begin{tabular}{|c|x{1.4cm}c}



\multirow{7}{*}{\rotatebox{90}{\textsc{MongoDB-O2}}}&\cellcolor{steel!30}\textbf{.74 ($<$.001)}& \quart{42.52}{27.37}{56.21}{100} \\ 
&\cellcolor{steel!30}{.51 ($=$.860)}& \quart{22.67}{39.44}{42.39}{100} \\ 
&\cellcolor{steel!30}\textbf{.71 ($<$.001)}& \quart{34.83}{26.82}{48.24}{100} \\ 
&\cellcolor{steel!30}{.59 ($=$.117)}& \quart{48.15}{51.85}{74.07}{100} \\ 
&\cellcolor{steel!30}{.56 ($=$.319)}& \quart{27.01}{38.88}{46.45}{100} \\ 
&-& \bquart{0.00}{35.46}{17.73}{100} \\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular}
 
    \vspace{0.05cm}
        \\ \midrule
               
              
     
            \begin{tabular}{l|c|x{1.4cm}c}
    



IRACE&\multirow{7}{*}{\rotatebox{90}{\textsc{x264-O1}}}&\cellcolor{steel!30}\textbf{.98 ($<$.001)}& \quart{34.93}{0.00}{34.93}{100} \\ 
GA&&\cellcolor{steel!30}{.51 ($=$.885)}& \quart{2.42}{2.94}{3.89}{100} \\ 
RS&&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}& \quart{100.00}{0.00}{100.00}{100} \\ 
MMO&&\cellcolor{red!10}{.44 ($=$.293)}& \bquart{0.28}{3.72}{2.14}{100} \\ 
PMO&&\cellcolor{red!10}{.49 ($=$.823)}& \quart{0.00}{5.12}{2.56}{100} \\ 
AdMMO&&-& \quart{0.63}{3.84}{2.55}{100} \\ 
&&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
  \begin{tabular}{|c|x{1.4cm}c}

 

\multirow{7}{*}{\rotatebox{90}{\textsc{x264-O2}}}&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}& \quart{8.37}{0.00}{8.37}{100} \\ 
&\cellcolor{steel!30}\textbf{.72 ($<$.001)}& \quart{1.57}{0.61}{1.87}{100} \\ 
&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}& \quart{100.00}{0.00}{100.00}{100} \\ 
&\cellcolor{steel!30}\textbf{.71 ($<$.001)}& \quart{1.33}{0.36}{1.51}{100} \\ 
&\cellcolor{steel!30}\textbf{.68 ($=$.003)}& \quart{0.76}{0.73}{1.13}{100} \\ 
&-& \bquart{0.00}{0.71}{0.35}{100} \\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
         &
   \begin{tabular}{|c|x{1.4cm}c}



\multirow{7}{*}{\rotatebox{90}{\textsc{LLVM-O1}}}&\cellcolor{steel!30}\textbf{.99 ($<$.001)}& \quart{81.46}{8.76}{85.84}{100} \\ 
&{.50 ($=$1.00)}& \bquart{0.00}{0.00}{0.00}{100} \\ 
&\cellcolor{steel!30}\textbf{.99 ($<$.001)}& \quart{92.48}{7.52}{96.24}{100} \\ 
&{.50 ($=$1.00)}& \bquart{0.00}{0.00}{0.00}{100} \\ 
&\cellcolor{steel!30}{.57 ($=$.228)}& \quart{1.72}{4.14}{3.79}{100} \\ 
&-& \bquart{0.00}{0.00}{0.00}{100} \\ 

&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
         &
  \begin{tabular}{|c|x{1.4cm}c}



\multirow{7}{*}{\rotatebox{90}{\textsc{LLVM-O2}}}&\cellcolor{steel!30}\textbf{.67 ($=$.004)}& \quart{57.21}{29.10}{71.76}{100} \\ 
&\cellcolor{steel!30}\textbf{.64 ($=$.020)}& \quart{44.28}{25.28}{56.91}{100} \\ 
&\cellcolor{steel!30}\textbf{.71 ($<$.001)}& \quart{71.25}{28.75}{85.63}{100} \\ 
&\cellcolor{steel!30}\textbf{.66 ($=$.007)}& \quart{33.76}{19.40}{43.47}{100} \\ 
&\cellcolor{steel!30}\textbf{.78 ($<$.001)}& \quart{64.79}{14.74}{72.16}{100} \\ 
&-& \bquart{0.00}{16.51}{8.26}{100} \\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
       
      &
        
         \begin{tabular}{p{1.3cm}ccc}
            \textbf{AdMMO vs.}   &   \textbf{$\#$ Win}& \textbf{$\#$ Lose} & \textbf{$\#$ Tie}   \\
            \hline
IRACE&13 (93\%)&1 (7\%)&0 (0\%)\\ 
GA&10 (72\%)&1 (7\%)&3 (21\%)\\ 
RS&14 (100\%)&0 (0\%)&0 (0\%)\\ 
MMO&10 (72\%)&2 (14\%)&2 (14\%)\\ 
PMO&12 (86\%)&2 (14\%)&0 (0\%)\\ \hline
\multicolumn{4}{c}{\textbf{Overall win/lose/tie for AdMMO}}\\ 

        \end{tabular}  
        
      % \vspace{0.05cm}
        %\\ \bottomrule
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/rq1-2.tex <==


% CS Table for RQ2
\begin{table*}[t!]
\caption{Comparing AdMMO with the state-of-the-art model-based optimizers over 50 runs. Formats are the same as Table~\ref{tb:rq1-1}. Tables of raw results throughout the tuning can be found at: \href{https://github.com/3c23/admmo/blob/main/supp-data.pdf}{\texttt{\textcolor{blue}{https://github.com/3c23/admmo/blob/main/supp-data.pdf}}}.}
    \label{tb:rq1-2}
    \footnotesize
    \setlength{\tabcolsep}{0.85mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc@{}cc}
            \begin{tabular}{l|c|cc}
            \cellcolor[gray]{1}\textbf{}  && \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


FLASH&\multirow{5}{*}{\rotatebox{90}{\textsc{MariaDB-O1}}}&\cellcolor{steel!30}\textbf{.84 ($<$.001)}& \quart{79.19}{20.81}{89.60}{100} \\ 
BOCA&&\cellcolor{steel!30}\textbf{.89 ($<$.001)}& \quart{73.23}{12.03}{79.25}{100} \\ 
AdMMO&&-& \bquart{0.00}{11.52}{5.76}{100} \\ 

&&&\\ 
&&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
          \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline
%&\cellcolor{steel!30}\textbf{.70 ($<$.001)}& \quart{56.14}{17.54}{64.92}{100} \\ 
%&\cellcolor{steel!30}\textbf{.64 ($=$.013)}& \quart{65.81}{34.19}{82.90}{100} \\ 
%&-& \bquart{0.00}{38.99}{19.49}{100} \\ 

\multirow{5}{*}{\rotatebox{90}{\textsc{MariaDB-O2}}}&\cellcolor{steel!30}\textbf{.69 ($<$.001)}& \quart{57.89}{16.84}{66.32}{100} \\ 
&\cellcolor{steel!30}\textbf{.66 ($=$.007)}& \quart{67.17}{32.83}{83.59}{100} \\ 
&-& \bquart{0.00}{33.76}{16.88}{100} \\ 

&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
         \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


\multirow{5}{*}{\rotatebox{90}{\textsc{Storm-O1}}}&\cellcolor{steel!30}\textbf{.87 ($<$.001)}& \quart{83.05}{16.95}{91.53}{100} \\ 
&\cellcolor{steel!30}\textbf{.75 ($<$.001)}& \quart{34.93}{16.85}{43.35}{100} \\ 
&-& \bquart{0.00}{15.85}{7.93}{100} \\ 

&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
              \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


\multirow{5}{*}{\rotatebox{90}{\textsc{Storm-O2}}}&\cellcolor{steel!30}\textbf{.93 ($<$.001)}& \quart{83.30}{16.70}{91.65}{100} \\ 
&\cellcolor{steel!30}\textbf{.90 ($<$.001)}& \quart{66.26}{16.82}{74.67}{100} \\ 
&-& \bquart{0.00}{7.97}{3.98}{100} \\ 
&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
            \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


%&{.50 ($=$.964)}& \quart{5.13}{14.87}{12.56}{100} \\ 
%&\cellcolor{red!10}{.49 ($=$.847)}& \bquart{0.00}{15.81}{7.90}{100} \\ 
%&-& \quart{50.90}{49.10}{75.45}{100} \\ 


\multirow{5}{*}{\rotatebox{90}{\textsc{VP9-O1}}}&{.50 ($=$.948)}& \quart{43.64}{56.36}{71.82}{100} \\ 
&\cellcolor{red!10}{.47 ($=$.593)}& \quart{24.21}{59.92}{54.17}{100} \\ 
&-& \bquart{0.00}{80.10}{40.05}{100} \\ 

&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular}  


   \vspace{0.05cm}
        \\ \midrule

         \begin{tabular}{l|c|x{1.4cm}c}


%FLASH&\cellcolor{steel!30}{.52 ($=$.777)}& \quart{7.02}{7.17}{10.60}{100} \\ 
%BOCA&\cellcolor{red!10}{.45 ($=$.354)}& \bquart{0.00}{7.61}{3.81}{100} \\ 
%AdMMO&-& \quart{41.78}{58.22}{70.89}{100} \\ 


FLASH&\multirow{5}{*}{\rotatebox{90}{\textsc{VP-O2}}}&\cellcolor{steel!30}{.53 ($=$.622)}& \quart{15.66}{16.01}{23.66}{100} \\ 
BOCA&&\cellcolor{red!10}{.47 ($=$.598)}& \bquart{0.00}{16.99}{8.50}{100} \\ 
AdMMO&&-& \quart{20.21}{79.79}{60.10}{100} \\ 


&&&\\ 
&&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
    \begin{tabular}{|c|x{1.4cm}c}


\multirow{5}{*}{\rotatebox{90}{\textsc{Keras-O1}}}&\cellcolor{steel!30}{.58 ($=$.143)}& \quart{72.30}{27.70}{86.15}{100} \\ 
&\cellcolor{steel!30}{.57 ($=$.252)}& \quart{34.07}{43.92}{56.03}{100} \\ 
&-& \bquart{0.00}{49.08}{24.54}{100} \\ 
&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
      \begin{tabular}{|c|x{1.4cm}c}
%&\cellcolor{steel!30}\textbf{.96 ($<$.001)}& \quart{75.53}{24.47}{87.77}{100} \\ 
%&\cellcolor{steel!30}\textbf{.86 ($<$.001)}& \quart{30.39}{23.21}{41.99}{100} \\ 
%&-& \bquart{0.00}{0.93}{0.47}{100} \\ 


\multirow{5}{*}{\rotatebox{90}{\textsc{Keras-O2}}}&\cellcolor{steel!30}\textbf{.94 ($<$.001)}& \quart{74.72}{25.28}{87.36}{100} \\ 
&\cellcolor{steel!30}\textbf{.82 ($<$.001)}& \quart{28.07}{23.98}{40.07}{100} \\ 
&-& \bquart{0.00}{35.55}{17.78}{100} \\ 
&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
    \begin{tabular}{|c|x{1.4cm}c}

%&\cellcolor{red!10}\textbf{.24 ($<$.001)}& \quart{19.50}{13.21}{26.11}{100} \\ 
%&\cellcolor{red!10}\textbf{.20 ($<$.001)}& \bquart{0.00}{11.30}{5.65}{100} \\ 
%&-& \quart{79.42}{20.58}{89.71}{100} \\ 



\multirow{5}{*}{\rotatebox{90}{\textsc{MongoDB-O1}}}&\cellcolor{red!10}\textbf{.18 ($<$.001)}& \quart{43.61}{29.54}{58.38}{100} \\ 
&\cellcolor{red!10}\textbf{.14 ($<$.001)}& \bquart{0.00}{25.27}{12.63}{100} \\ 
&-& \quart{40.79}{59.21}{70.39}{100} \\ 

&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
      \begin{tabular}{|c|x{1.4cm}c}

%&\cellcolor{red!10}\textbf{.23 ($<$.001)}& \quart{1.31}{9.48}{6.05}{100} \\ 
%&\cellcolor{red!10}\textbf{.22 ($<$.001)}& \bquart{0.00}{6.77}{3.39}{100} \\ 
%&-& \quart{78.31}{21.69}{89.15}{100} \\ 

\multirow{5}{*}{\rotatebox{90}{\textsc{MongoDB-O2}}}&\cellcolor{red!10}\textbf{.14 ($<$.001)}& \quart{5.64}{40.82}{26.05}{100} \\ 
&\cellcolor{red!10}\textbf{.14 ($<$.001)}& \bquart{0.00}{29.17}{14.59}{100} \\ 
&-& \quart{21.95}{78.05}{60.98}{100} \\ 

&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular}

   \vspace{0.05cm}
        \\ \midrule

               
              
     
          \begin{tabular}{l|c|x{1.4cm}c}
   
     


FLASH&\multirow{4}{*}{\rotatebox{90}{\textsc{x264-O1}}}&\cellcolor{steel!30}\textbf{.87 ($<$.001)}& \quart{4.00}{6.10}{7.05}{100} \\ 
BOCA&&\cellcolor{steel!30}\textbf{.73 ($<$.001)}& \quart{50.06}{49.94}{75.03}{100} \\ 
AdMMO&&-& \bquart{2.07}{5.20}{4.67}{100} \\ 
&&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
      \begin{tabular}{|c|x{1.4cm}c}




\multirow{4}{*}{\rotatebox{90}{\textsc{x264-O2}}}&\cellcolor{steel!30}\textbf{.82 ($<$.001)}& \quart{3.00}{4.58}{5.29}{100} \\ 
&\cellcolor{steel!30}\textbf{.89 ($<$.001)}& \quart{71.27}{28.73}{85.64}{100} \\ 
&-& \bquart{4.75}{0.81}{5.15}{100} \\ 

&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
         &
      \begin{tabular}{|c|x{1.4cm}c}

\multirow{4}{*}{\rotatebox{90}{\textsc{LLVM-O1}}}&\cellcolor{steel!30}\textbf{.97 ($<$.001)}& \quart{89.02}{10.98}{94.51}{100} \\ 
&\cellcolor{steel!30}\textbf{.98 ($<$.001)}& \quart{90.40}{9.13}{94.97}{100} \\ 
&-& \bquart{0.00}{7.51}{3.76}{100} \\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
         &
      \begin{tabular}{|c|x{1.4cm}c}


\multirow{4}{*}{\rotatebox{90}{\textsc{LLVM-O2}}}&\cellcolor{steel!30}\textbf{.69 ($<$.001)}& \quart{63.52}{29.50}{78.27}{100} \\ 
&\cellcolor{steel!30}\textbf{.68 ($=$.001)}& \quart{69.31}{30.69}{84.65}{100} \\ 
&-& \bquart{0.00}{29.37}{14.68}{100} \\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
       
      &
        
 
     
             
         \begin{tabular}{p{1.3cm}ccc}
            \textbf{AdMMO vs.}   &   \textbf{$\#$ Win}& \textbf{$\#$ Lose} & \textbf{$\#$ Tie}   \\
            \hline
FLASH&11 (79\%)&2 (14\%)&1 (7\%)\\ 
BOCA&10 (72\%)&4 (28\%)&0 (0\%)\\  \hline
\multicolumn{4}{c}{\textbf{Overall win/lose/tie for AdMMO}}\\ 

        \end{tabular}  
        
        
        \\
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/rq1-bk.tex <==


% CS Table for RQ2
\begin{table*}[t!]
\caption{Comparing MOO$+$ with the other state-of-the-arts over 50 runs. SO$_{best}$ and MMO$_{best}$ denote the best single-objective optimizer and the MMO model with the best weight, respectively. \quartexp{0}{20}{10}{20} shows the average and standard error on the target performance objective achieved (all objective values are normalized within $[0,1]$ and the closer to the left, the better). \bquartexp{0}{20}{10}{20} denote the best average among others. Column ``$\hat{A}_{12}$ ($p$ value)'' shows the $\hat{A}_{12}$ and $p$ value when comparing the corresponding counterpart with MOO$+$. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} denote MMO$+$ wins while \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red cells} mean it loses; otherwise it is a tie. The statistically significant comparisons, i.e., $\hat{A}_{12} \geq 0.56$ (or $\hat{A}_{12} \leq 0.44$) and $p<0.05$ are highlighted in bold.}
    \label{tb:rq1}
    \footnotesize
    \setlength{\tabcolsep}{0.85mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc}
        \begin{tabular}{lclc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (Standard Error)}}  \\
            \hline
IRACE&\cellcolor{steel!30}\textbf{.88 ($<$.001)}&3462.99 (7.92)& \quart{82.73}{17.27}{91.36}{100} \\ 
GA&\cellcolor{steel!30}\textbf{.67 ($=$.003)}&3406.17 (4.65)& \quart{24.34}{10.14}{29.41}{100} \\ 
RS&\cellcolor{steel!30}\textbf{.86 ($<$.001)}&3439.29 (5.73)& \quart{59.28}{12.49}{65.52}{100} \\ 
MMO&\cellcolor{steel!30}\textbf{.62 ($=$.044)}&3399.65 (4.66)& \quart{17.22}{10.17}{22.31}{100} \\ 
PMO&\cellcolor{steel!30}\textbf{.64 ($=$.018)}&3400.77 (4.92)& \quart{18.16}{10.73}{23.52}{100} \\ 
AdMMO&-&3383.18 (3.98)& \bquart{0.00}{8.69}{4.34}{100} \\ 
        \end{tabular} & 
        &
       \begin{tabular}{lclcl}
                  \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (Standard Error)}}  \\
            \hline
&\cellcolor{steel!30}{.56 ($=$.284)}&1.05 (0.01)& \quart{48.00}{26.89}{61.44}{100} \\ 
&\cellcolor{red!10}{.39 ($=$.066)}&1.01 (0.01)& \quart{2.53}{13.24}{9.15}{100} \\ 
&\cellcolor{steel!30}\textbf{.66 ($=$.006)}&1.06 (0.01)& \quart{62.23}{25.60}{75.03}{100} \\ 
&\cellcolor{red!10}{.40 ($=$.089)}&1.00 (0.01)& \bquart{0.00}{14.26}{7.13}{100} \\ 
&\cellcolor{steel!30}\textbf{.65 ($=$.010)}&1.07 (0.01)& \quart{71.16}{28.84}{85.58}{100} \\ 
&-&1.02 (0.00)& \quart{17.08}{12.37}{23.27}{100} \\ 
        \end{tabular} &
        &
       \begin{tabular}{lclcl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (Standard Error)}}  \\
            \hline
&\cellcolor{steel!30}\textbf{.84 ($<$.001)}&33556 (170)& \quart{0.00}{25.30}{12.65}{100} \\ 
&\cellcolor{steel!30}\textbf{.76 ($<$.001)}&34579 (22)& \quart{86.96}{3.26}{88.59}{100} \\ 
&\cellcolor{steel!30}\textbf{.87 ($<$.001)}&33678 (135)& \quart{11.69}{20.02}{21.70}{100} \\ 
&\cellcolor{steel!30}\textbf{.70 ($<$.001)}&34615 (21)& \quart{89.75}{3.14}{91.32}{100} \\ 
&\cellcolor{steel!30}\textbf{.87 ($<$.001)}&34558 (16)& \quart{85.91}{2.33}{87.07}{100} \\ 
&-&34722 (11)& \bquart{98.40}{1.60}{99.20}{100} \\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (Standard Error)}}  \\
            \hline

&\cellcolor{steel!30}\textbf{.98 ($<$.001)}&206.37 (0.56)& \quart{78.23}{13.01}{84.73}{100} \\ 
&{.50 ($=$1.00)}&199.03 (0.00)& \bquart{0.00}{0.00}{0.00}{100} \\ 
&\cellcolor{steel!30}\textbf{.97 ($<$.001)}&206.91 (0.78)& \quart{82.03}{17.97}{91.02}{100} \\ 
&{.50 ($=$1.00)}&199.03 (0.00)& \bquart{0.00}{0.00}{0.00}{100} \\ 
&\cellcolor{steel!30}{.59 ($=$.121)}&200.26 (0.52)& \quart{8.21}{11.95}{14.18}{100} \\ 
&-&199.03 (0.00)& \bquart{0.00}{0.00}{0.00}{100} \\ 
        \end{tabular}  
        \\
            (a). \textsc{MariaDB-O1}; Runtime (s)&& (b). \textsc{MariaDB-O2}; CPU load && (c). \textsc{Storm-O1}; Throughput (msgs/min)&& (d). \textsc{Storm-O2}; Latency (min)


        \\
        \\
             \begin{tabular}{lclc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (SE)}}  \\
            \hline
IRACE&\cellcolor{steel!30}\textbf{.98 ($<$.001)}&31168 (790.1)& \quart{30.91}{26.09}{43.96}{100} \\ 
GA&\cellcolor{steel!30}\textbf{.66 ($=$.005)}&28545 (7.4)& \quart{0.52}{0.24}{0.64}{100} \\ 
RS&\cellcolor{steel!30}\textbf{.98 ($<$.001)}&30661 (661.8)& \quart{24.67}{21.86}{35.60}{100} \\ 
MMO&\cellcolor{steel!30}\textbf{.64 ($=$.018)}&28542 (7.9)& \quart{0.46}{0.26}{0.59}{100} \\ 
PMO&\cellcolor{steel!30}\textbf{.87 ($<$.001)}&33167 (1394.1)& \quart{53.96}{46.04}{76.98}{100} \\ 
AdMMO&-&28513 (7.35)& \bquart{0.00}{0.24}{0.12}{100} \\ 
        \end{tabular} & 
        &
       \begin{tabular}{lclcl}
                  \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (SE)}}  \\
            \hline
&\cellcolor{steel!30}\textbf{.74 ($<$.001)}&3.48 (0.00)& \quart{35.34}{7.52}{39.10}{100} \\ 
&\cellcolor{red!10}{.43 ($=$.255)}&3.43 (0.00)& \bquart{0.00}{2.70}{1.35}{100} \\ 
&\cellcolor{steel!30}\textbf{.80 ($<$.001)}&3.49 (0.00)& \quart{42.54}{5.54}{45.32}{100} \\ 
&\cellcolor{red!10}{.49 ($=$.844)}&3.45 (0.01)& \quart{8.04}{11.48}{13.78}{100} \\ 
&\cellcolor{steel!30}\textbf{.77 ($<$.001)}&3.54 (0.01)& \quart{75.91}{24.09}{87.95}{100} \\ 
&-&3.46 (0.01)& \quart{15.79}{13.30}{22.45}{100} \\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (SE)}}  \\
            \hline
&\cellcolor{red!10}{.47 ($=$.591)}&0.69 (0.01)& \quart{35.01}{16.95}{43.48}{100} \\ 
&\cellcolor{steel!30}\textbf{.63 ($=$.026)}&0.63 (0.01)& \quart{0.00}{15.34}{7.67}{100} \\ 
&\cellcolor{steel!30}{.55 ($=$.404)}&0.67 (0.01)& \quart{18.04}{18.10}{27.09}{100} \\ 
&\cellcolor{steel!30}\textbf{.62 ($=$.038)}&0.64 (0.01)& \quart{1.92}{14.95}{9.40}{100} \\ 
&\cellcolor{red!10}\textbf{.23 ($<$.001)}&0.79 (0.00)& \bquart{100.00}{0.00}{100.00}{100} \\ 
&-&0.68 (0.01)& \quart{27.63}{17.04}{36.15}{100} \\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (SE)}}  \\
            \hline
&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&412.82 (1.40)& \quart{79.45}{20.55}{89.72}{100} \\ 
&\cellcolor{steel!30}\textbf{.73 ($<$.001)}&401.30 (0.10)& \quart{4.40}{1.49}{5.15}{100} \\ 
&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&410.16 (0.86)& \quart{63.91}{12.59}{70.21}{100} \\ 
&\cellcolor{steel!30}\textbf{.64 ($=$.016)}&401.08 (0.11)& \quart{2.78}{1.59}{3.58}{100} \\ 
&\cellcolor{steel!30}\textbf{.66 ($=$.005)}&401.08 (0.09)& \quart{2.91}{1.29}{3.56}{100} \\ 
&-&400.67 (0.07)& \bquart{0.00}{1.05}{0.52}{100} \\ 

        \end{tabular}  
        \\
            (e). \textsc{VP9-O1}; Runtime (s)&& (f). \textsc{VP9-O2}; CPU load && (g). \textsc{Keras/DNN-O1}; AUC&& (h). \textsc{Keras/DNN-O2}; Inference Time (ms)
        \\
        
               \\
               
                  \begin{tabular}{lccc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (SE)}}  \\
            \hline
IRACE&\cellcolor{steel!30}\textbf{.73 ($<$.001)}&3934.81 (55.23)& \quart{52.60}{28.40}{66.80}{100} \\ 
GA&\cellcolor{steel!30}\textbf{.63 ($=$.023)}&3753.71 (39.23)& \quart{10.15}{20.17}{20.24}{100} \\ 
RS&\cellcolor{steel!30}\textbf{.78 ($<$.001)}&3998.31 (65.64)& \quart{66.25}{33.75}{83.12}{100} \\ 
MMO&\cellcolor{steel!30}\textbf{.64 ($=$.018)}&3797.74 (49.84)& \quart{18.75}{25.63}{31.56}{100} \\ 
PMO&\cellcolor{steel!30}\textbf{.64 ($=$.017)}&3780.82 (37.87)& \quart{17.47}{19.47}{27.21}{100} \\ 
AdMMO&-&3723.14 (48.15)& \bquart{0.00}{24.76}{12.38}{100} \\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                  \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (SE)}}  \\
            \hline
&\cellcolor{steel!30}\textbf{.76 ($<$.001)}&31.71 (0.48)& \quart{68.95}{31.05}{84.47}{100} \\ 
&\cellcolor{steel!30}{.54 ($=$.482)}&30.10 (0.31)& \quart{22.53}{19.87}{32.46}{100} \\ 
&\cellcolor{steel!30}\textbf{.73 ($<$.001)}&31.43 (0.47)& \quart{60.21}{30.43}{75.43}{100} \\ 
&\cellcolor{steel!30}{.61 ($=$.051)}&30.08 (0.34)& \quart{21.25}{21.56}{32.03}{100} \\ 
&\cellcolor{steel!30}{.58 ($=$.196)}&30.25 (0.30)& \quart{27.86}{18.99}{37.36}{100} \\ 
&-&29.43 (0.35)& \bquart{0.00}{22.29}{11.14}{100} \\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                 \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (SE)}}  \\
            \hline
&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&51.84 (0.00)& \quart{65.07}{0.00}{65.07}{100} \\ 
&\cellcolor{red!10}{.48 ($=$.705)}&54.20 (0.12)& \bquart{96.01}{3.18}{97.60}{100} \\ 
&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&47.12 (0.00)& \quart{0.00}{0.00}{0.00}{100} \\ 
&\cellcolor{steel!30}{.53 ($=$.659)}&54.07 (0.14)& \quart{93.91}{3.76}{95.79}{100} \\ 
&\cellcolor{red!10}{.44 ($=$.328)}&54.19 (0.19)& \quart{94.88}{5.12}{97.44}{100} \\ 
&-&54.09 (0.12)& \quart{94.43}{3.42}{96.15}{100} \\ 

        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (SE)}}  \\
            \hline
&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&404.44 (0.00)& \quart{8.14}{0.00}{8.14}{100} \\ 
&\cellcolor{steel!30}\textbf{.71 ($<$.001)}&357.59 (2.18)& \quart{1.32}{0.61}{1.62}{100} \\ 
&\cellcolor{steel!30}\textbf{1.0 ($<$.001)}&1064.83 (0.00)& \quart{100.00}{0.00}{100.00}{100} \\ 
&\cellcolor{steel!30}\textbf{.72 ($<$.001)}&355.00 (1.31)& \quart{1.08}{0.36}{1.26}{100} \\ 
&\cellcolor{steel!30}\textbf{.70 ($<$.001)}&352.28 (2.65)& \quart{0.51}{0.74}{0.88}{100} \\ 
&-&347.58 (1.63)& \bquart{0.00}{0.45}{0.23}{100} \\ 
        \end{tabular}  
        \\
            (i). \textsc{MongoDB-O1}; Runtime (min)&& (j). \textsc{MongoDB-O2}; CPU load && (k). \textsc{x264-O1}; Iterations&& (l). \textsc{x264-O2}; Energy (J)
        \\
        
               \\
     
           \begin{tabular}{lcccl}
                  \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (SE)}}  \\
            \hline
     
IRACE&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&938.32 (3.41)& \quart{81.46}{8.76}{85.84}{100} \\ 
GA&{.50 ($=$1.00)}&871.42 (0.00)& \bquart{0.00}{0.00}{0.00}{100} \\ 
RS&\cellcolor{steel!30}\textbf{.99 ($<$.001)}&946.43 (2.93)& \quart{92.48}{7.52}{96.24}{100} \\ 
MMO&{.50 ($=$1.00)}&871.42 (0.00)& \bquart{0.00}{0.00}{0.00}{100} \\ 
PMO&\cellcolor{steel!30}{.57 ($=$.228)}&874.38 (1.61)& \quart{1.72}{4.14}{3.79}{100} \\ 
AdMMO&-&871.42 (0.00)& \bquart{0.00}{0.00}{0.00}{100} \\       
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                  \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\hat{A}_{12}$ ($p$ value)} &
            \multicolumn{2}{c}{\cellcolor[gray]{1}\textbf{Mean (SE)}}  \\
            \hline
&\cellcolor{steel!30}\textbf{.67 ($=$.004)}&25.36 (0.01)& \quart{58.15}{28.46}{72.38}{100} \\ 
&\cellcolor{steel!30}\textbf{.65 ($=$.011)}&25.35 (0.01)& \quart{45.51}{24.72}{57.87}{100} \\ 
&\cellcolor{steel!30}\textbf{.70 ($<$.001)}&25.37 (0.01)& \quart{71.89}{28.11}{85.94}{100} \\ 
&\cellcolor{steel!30}\textbf{.65 ($=$.009)}&25.34 (0.01)& \quart{35.23}{18.97}{44.71}{100} \\ 
&\cellcolor{steel!30}\textbf{.74 ($<$.001)}&25.36 (0.01)& \quart{65.57}{14.42}{72.78}{100} \\ 
&-&25.31 (0.01)& \bquart{0.00}{20.90}{10.45}{100} \\ 
        \end{tabular} &
      
        
             \begin{minipage}{0.001\textwidth}
             \vspace{0.04cm}
         \begin{tabular}{p{7.65cm}ccc}
              &   \textbf{\% Win}& \textbf{\% Lose} & \textbf{\% Tie}   \\
            \hline
AdMMO versus IRACE&100\%&0\%&0\%\\ 
AdMMO versus GA&65\%&21\%&14\%\\ 
AdMMO versus RS&100\%&0\%&0\%\\ 
AdMMO versus MMO&72\%&14\%&14\%\\ 
AdMMO versus PMO&86\%&14\%&0\%\\ 
&&&\\ 
        \end{tabular}    
     \end{minipage}
        
        &
  
        &
   
         &
         
                
       \\
            (m). \textsc{LLVM-O1}; Runtime (min)&& (n). \textsc{LLVM-O2}; CPU load  & \begin{minipage}{0.001\textwidth}
                        \begin{tabular}{c}
           (o). Overall \% win/loss/tie for AdMMO versus the others
        \end{tabular} 
                 \end{minipage}&
                 &&
        \\
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/rq3.tex <==


% CS Table for RQ2
\begin{table*}[t!]
\caption{Ablation analysis of AdMMO over 50 runs. Formats are the same as Table~\ref{tb:rq1-1}.}
    \label{tb:rq3}
    \footnotesize
    \setlength{\tabcolsep}{0.85mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc@{}cc}
            \begin{tabular}{l|c|cc}
            \cellcolor[gray]{1}\textbf{}  && \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


AdMMO$_c$&\multirow{5}{*}{\rotatebox{90}{\textsc{MariaDB-O1}}}&\cellcolor{steel!30}{.58 ($=$.191)}& \quart{50.52}{42.04}{71.54}{100} \\ 
AdMMO$_d$&&\cellcolor{steel!30}{.58 ($=$.151)}& \quart{47.85}{52.15}{73.92}{100} \\ 
AdMMO&&-& \bquart{0.00}{44.55}{22.27}{100} \\ 
&&&\\ 
&&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
          \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline
%&\cellcolor{steel!30}\textbf{.70 ($<$.001)}& \quart{56.14}{17.54}{64.92}{100} \\ 
%&\cellcolor{steel!30}\textbf{.64 ($=$.013)}& \quart{65.81}{34.19}{82.90}{100} \\ 
%&-& \bquart{0.00}{38.99}{19.49}{100} \\ 


\multirow{5}{*}{\rotatebox{90}{\textsc{MariaDB-O2}}}&\cellcolor{steel!30}\textbf{.66 ($=$.006)}& \quart{76.73}{23.27}{88.36}{100} \\ 
&\cellcolor{red!10}\textbf{.35 ($=$.011)}& \bquart{0.00}{21.70}{10.85}{100} \\ 
&-& \quart{40.29}{18.65}{49.61}{100} \\ 

&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
         \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


\multirow{5}{*}{\rotatebox{90}{\textsc{Storm-O1}}}&\cellcolor{steel!30}{.53 ($=$.577)}& \quart{7.22}{13.09}{13.77}{100} \\ 
&\cellcolor{steel!30}\textbf{.86 ($<$.001)}& \quart{79.38}{20.62}{89.69}{100} \\ 
&-& \bquart{0.00}{8.46}{4.23}{100} \\ 
&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
              \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline
\multirow{5}{*}{\rotatebox{90}{\textsc{Storm-O2}}}&{.50 ($=$1.00)}& \bquart{0.00}{100.00}{50.00}{100} \\ 
&{.50 ($=$1.00)}& \bquart{0.00}{100.00}{50.00}{100} \\ 
&-& \bquart{0.00}{100.00}{50.00}{100} \\ 
&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
            \begin{tabular}{|c|cc}
            \cellcolor[gray]{1}\textbf{}  & \cellcolor[gray]{1}\textbf{$\mathbf{\hat{A}_{12}}$ (\textbf{p-value})} &
            \cellcolor[gray]{1}\textbf{Mean (SE)}  \\
            \hline


%&{.50 ($=$.964)}& \quart{5.13}{14.87}{12.56}{100} \\ 
%&\cellcolor{red!10}{.49 ($=$.847)}& \bquart{0.00}{15.81}{7.90}{100} \\ 
%&-& \quart{50.90}{49.10}{75.45}{100} \\ 


\multirow{5}{*}{\rotatebox{90}{\textsc{VP9-O1}}}&\cellcolor{steel!30}\textbf{.66 ($=$.005)}& \quart{22.00}{78.00}{61.00}{100} \\ 
&\cellcolor{steel!30}\textbf{.69 ($=$.001)}& \quart{2.09}{0.83}{2.51}{100} \\ 
&-& \bquart{0.00}{0.78}{0.39}{100} \\ 
&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular}  


   \vspace{0.05cm}
        \\ \midrule

         \begin{tabular}{l|c|x{1.4cm}c}


%FLASH&\cellcolor{steel!30}{.52 ($=$.777)}& \quart{7.02}{7.17}{10.60}{100} \\ 
%BOCA&\cellcolor{red!10}{.45 ($=$.354)}& \bquart{0.00}{7.61}{3.81}{100} \\ 
%AdMMO&-& \quart{41.78}{58.22}{70.89}{100} \\ 


AdMMO$_c$&\multirow{5}{*}{\rotatebox{90}{\textsc{VP-O2}}}&\cellcolor{steel!30}\textbf{.64 ($=$.014)}& \quart{63.44}{36.56}{81.72}{100} \\ 
AdMMO$_d$&&{.50 ($=$.962)}& \bquart{0.00}{14.09}{7.04}{100} \\ 
AdMMO&&-& \quart{21.65}{30.64}{36.97}{100} \\ 

&&&\\ 
&&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
    \begin{tabular}{|c|x{1.4cm}c}



\multirow{5}{*}{\rotatebox{90}{\textsc{Keras-O1}}}&\cellcolor{steel!30}\textbf{.63 ($=$.024)}& \quart{64.51}{30.11}{79.56}{100} \\ 
&\cellcolor{steel!30}\textbf{.65 ($=$.010)}& \quart{70.78}{29.22}{85.39}{100} \\ 
&-& \bquart{0.00}{34.34}{17.17}{100} \\ 
&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
      \begin{tabular}{|c|x{1.4cm}c}
%&\cellcolor{steel!30}\textbf{.96 ($<$.001)}& \quart{75.53}{24.47}{87.77}{100} \\ 
%&\cellcolor{steel!30}\textbf{.86 ($<$.001)}& \quart{30.39}{23.21}{41.99}{100} \\ 
%&-& \bquart{0.00}{0.93}{0.47}{100} \\ 


\multirow{5}{*}{\rotatebox{90}{\textsc{Keras-O2}}}&\cellcolor{steel!30}{.54 ($=$.478)}& \quart{23.08}{38.93}{42.55}{100} \\ 
&\cellcolor{steel!30}\textbf{.67 ($=$.003)}& \quart{68.30}{31.70}{84.15}{100} \\ 
&-& \bquart{0.00}{18.37}{9.19}{100} \\ 
&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
    \begin{tabular}{|c|x{1.4cm}c}

%&\cellcolor{red!10}\textbf{.24 ($<$.001)}& \quart{19.50}{13.21}{26.11}{100} \\ 
%&\cellcolor{red!10}\textbf{.20 ($<$.001)}& \bquart{0.00}{11.30}{5.65}{100} \\ 
%&-& \quart{79.42}{20.58}{89.71}{100} \\ 


\multirow{5}{*}{\rotatebox{90}{\textsc{MongoDB-O1}}}&\cellcolor{steel!30}\textbf{.70 ($<$.001)}& \quart{59.08}{40.92}{79.54}{100} \\ 
&\cellcolor{steel!30}\textbf{.67 ($=$.003)}& \quart{22.78}{44.82}{45.19}{100} \\ 
&-& \bquart{0.00}{47.06}{23.53}{100} \\ 
&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
      \begin{tabular}{|c|x{1.4cm}c}

%&\cellcolor{red!10}\textbf{.23 ($<$.001)}& \quart{1.31}{9.48}{6.05}{100} \\ 
%&\cellcolor{red!10}\textbf{.22 ($<$.001)}& \bquart{0.00}{6.77}{3.39}{100} \\ 
%&-& \quart{78.31}{21.69}{89.15}{100} \\ 

\multirow{5}{*}{\rotatebox{90}{\textsc{MongoDB-O2}}}&\cellcolor{steel!30}\textbf{.67 ($=$.003)}& \quart{39.50}{38.58}{58.79}{100} \\ 
&\cellcolor{steel!30}\textbf{.62 ($=$.036)}& \quart{49.36}{50.64}{74.68}{100} \\ 
&-& \bquart{0.00}{41.88}{20.94}{100} \\ 
&&\\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular}

   \vspace{0.05cm}
        \\ \midrule

               
              
     
          \begin{tabular}{l|c|x{1.4cm}c}
   
     


AdMMO$_c$&\multirow{4}{*}{\rotatebox{90}{\textsc{x264-O1}}}&\cellcolor{steel!30}\textbf{.66 ($=$.006)}& \quart{74.54}{25.46}{87.27}{100} \\ 
AdMMO$_d$&&{.50 ($=$.992)}& \quart{9.99}{24.48}{22.23}{100} \\ 
AdMMO&&-& \bquart{0.00}{27.82}{13.91}{100} \\ 
&&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
      \begin{tabular}{|c|x{1.4cm}c}


\multirow{4}{*}{\rotatebox{90}{\textsc{x264-O2}}}&\cellcolor{steel!30}\textbf{.63 ($=$.024)}& \quart{37.44}{40.52}{57.70}{100} \\ 
&\cellcolor{steel!30}\textbf{.65 ($=$.008)}& \quart{70.58}{29.42}{85.29}{100} \\ 
&-& \bquart{0.00}{51.72}{25.86}{100} \\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
         &
      \begin{tabular}{|c|x{1.4cm}c}

\multirow{4}{*}{\rotatebox{90}{\textsc{LLVM-O1}}}&{.50 ($=$1.00)}& \bquart{0.00}{100.00}{50.00}{100} \\ 
&{.50 ($=$1.00)}& \bquart{0.00}{100.00}{50.00}{100} \\ 
&-& \bquart{0.00}{100.00}{50.00}{100} \\ 
&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
         &
      \begin{tabular}{|c|x{1.4cm}c}


\multirow{4}{*}{\rotatebox{90}{\textsc{LLVM-O2}}}&\cellcolor{steel!30}\textbf{.64 ($=$.013)}& \quart{58.77}{32.27}{74.90}{100} \\ 
&\cellcolor{steel!30}\textbf{.66 ($=$.005)}& \quart{65.22}{34.78}{82.61}{100} \\ 
&-& \bquart{0.00}{23.18}{11.59}{100} \\ 

&&\squart{1}{1}{1}{100}\\ 
        \end{tabular} &
       
      &
        
 
     
             
         \begin{tabular}{p{1.3cm}ccc}
            \textbf{AdMMO vs.}   &   \textbf{$\#$ Win}& \textbf{$\#$ Lose} & \textbf{$\#$ Tie}   \\
            \hline
AdMMO$_c$&12 (86\%)&0 (0\%)&2 (14\%)\\ 
AdMMO$_d$&9 (65\%)&1 (7\%)&4 (28\%)\\   \hline
\multicolumn{4}{c}{\textbf{Overall win/lose/tie for AdMMO}}\\ 

        \end{tabular}  
        
        
        \\
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/sys-bk.tex <==
\begin{table}[t!]
\caption{Configurable software systems and performance objectives studied. $|\mathbfcal{O}|$ and $|\mathbfcal{S}|$ denote the number of options and search space, respectively. The references show the work that uses the system.}
\label{tb:sys}
%\setlength{\tabcolsep}{1mm}
\centering
%\footnotesize

  \begin{adjustbox}{max width = \columnwidth}

\begin{tabular}{llllrr}


\toprule
\textbf{System}&\textbf{Language}&\textbf{Domain}&\textbf{The Two Performance Objectives}&\textbf{$|\mathbfcal{O}|$}&\textbf{$|\mathbfcal{S}|$}\\

\midrule

{\textsc{MariaDB}~\cite{DBLP:journals/corr/abs-2112-07303}}&C/C$++$/Perl&{SQL database}&Runtime and CPU load&{10}&{864}\\


{\textsc{Storm}~\cite{nair2018finding,DBLP:conf/mascots/JamshidiC16,DBLP:conf/sigsoft/0001Chen21}}&Java/Clojure&{Stream process}&Throughput and Latency&{6}&{2,880}\\



{\textsc{VP9}~\cite{DBLP:journals/corr/abs-2112-07303}}&C&{Video encoding}&Runtime and CPU load&{12}&{3,008}\\




{\textsc{Keras}~\cite{DBLP:conf/mascots/MendesCRG20,DBLP:conf/sigsoft/JamshidiVKS18}}&Python&{Deep learning}&AUC and Inference time&{13}&{12,288}\\



{\textsc{MongoDB}~\cite{DBLP:journals/corr/abs-2112-07303}}&C$++$&{Non-SQL database}&Runtime and CPU load&{15}&{6,840}\\



{\textsc{x264}~\cite{nair2018finding,DBLP:conf/icse/SiegmundKKABRS12,DBLP:conf/sigsoft/0001Chen21}}&C&{Video encoding}&PSNR and Energy consumption&{17}&{53,662}\\



{\textsc{LLVM}~\cite{nair2018finding,DBLP:journals/corr/abs-2112-07303}}&C$++$&{Compiler}&Runtime and CPU load&{16}&{65,436}\\


% \textsc{MariaDB}~\cite{DBLP:journals/corr/abs-2112-07303}&SQL database&\textsc{O1:} runtime& \textsc{O2:} CPU load&10&864\\

% \textsc{Storm}~\cite{nair2018finding,DBLP:conf/mascots/JamshidiC16,DBLP:conf/sigsoft/0001Chen21}&stream process&\textsc{O1:} throughput& \textsc{O2:} latency&6&2,880\\


% \textsc{VP9}~\cite{DBLP:journals/corr/abs-2112-07303}&video encoding&\textsc{O1:} runtime& \textsc{O2:} CPU load&12&3,008\\


% \textsc{MongoDB}~\cite{DBLP:journals/corr/abs-2112-07303}&no-SQL database&\textsc{O1:} runtime& \textsc{O2:} CPU load&15&6,840\\

% \textsc{Keras}~\cite{DBLP:conf/mascots/MendesCRG20,DBLP:conf/sigsoft/JamshidiVKS18}&deep learning&\textsc{O1:} AUC& \textsc{O2:} inferred time&13&12,288\\



% \textsc{x264}~\cite{nair2018finding,DBLP:conf/icse/SiegmundKKABRS12,DBLP:conf/sigsoft/0001Chen21}&video encoding&\textsc{O1:} PSNR& \textsc{O2:} energy usage&17&53,662\\


% \textsc{LLVM}~\cite{nair2018finding,DBLP:journals/corr/abs-2112-07303}&compiler&\textsc{O1:} runtime& \textsc{O2:} CPU load&16&65,436\\
\bottomrule


%1.92$\times 10^{10}$


\end{tabular}
  \end{adjustbox}
  %\vspace{-0.4cm}
\end{table}
